The Emergence of Reproducibility and Generalizability in Diffusion Models

In this work, we investigate an intriguing and prevalent phenomenon of diffusion models which we term as "consistent model reproducibility": given the same starting noise input and a deterministic sampler, different diffusion models often yield remarkably similar outputs. We confirm this phenomenon through comprehensive experiments, implying that different diffusion models consistently reach the same data distribution and scoring function regardless of diffusion model frameworks, model architectures, or training procedures. More strikingly, our further investigation implies that diffusion models are learning distinct distributions affected by the training data size. This is supported by the fact that the model reproducibility manifests in two distinct training regimes: (i) "memorization regime", where the diffusion model overfits to the training data distribution, and (ii) "generalization regime", where the model learns the underlying data distribution. Our study also finds that this valuable property generalizes to many variants of diffusion models, including those for conditional use, solving inverse problems, and model fine-tuning. Finally, our work raises numerous intriguing theoretical questions for future investigation and highlights practical implications regarding training efficiency, model privacy, and the controlled generation of diffusion models.

==> Marcos/macro.tex <==
\usepackage{tgpagella}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}
\usepackage[hidelinks]{hyperref}
\usepackage{amsmath,amsthm,amssymb,amsbsy,amsfonts,amscd,bm}
\usepackage{paralist}
\usepackage{xcolor}
\usepackage{color}
\usepackage{graphicx}
\graphicspath{{./figs/}}
\usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{comment}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{fancyhdr}
\usepackage{authblk}
%\usepackage{cite}
%\usepackage{citesort}
\usepackage{cleveref}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{bbding}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{bbold}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{cleveref}
\usepackage{enumitem}
\usepackage{tcolorbox}
% \usepackage{subfigure}
\usepackage{bbding}
% \usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
\usepackage{titletoc}
\usepackage{titlesec}
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\usepackage[toc, page]{appendix}
\usepackage[numbers]{natbib} 
% Theorems
\def \remarks {\noindent {\bf Remarks.}\ \ }
% \newtheorem{thm}{Theorem}%[section] %(If you want theorem numbered
\newtheorem{lemma}{Lemma}%[section] %%    with section number.
\newtheorem{coro}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]
\newtheorem{definition}{Definition}%[section]
\newtheorem{defi}{Definition}%[section]
\newtheorem{assum}{Assumption}
\newtheorem*{goal}{Plan}
% \newtheorem{theorem}{Theorem}
\newtheorem{lem}{Lemma}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
% \theoremstyle{problem}
\newtheorem{problem}{Problem}

% fields
\renewcommand{\O}{\mathbb{O}}
\newcommand{\R}{\mathbb{R}}
\def \real    { \mathbb{R} }
\def \reals   { \mathbb{R} }
\def \Real {\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\def \complex{\mathbb{C}}
\def \Complex {\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

%%%
\newcommand{\xiao}[1]{{\color{magenta}{\bf Xiao: #1}}}
%%%
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\en}{\begin{equation*}}
\newcommand{\een}{\end{equation*}}
\newcommand{\eqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bmat}{\begin{bmatrix}}
\newcommand{\emat}{\end{bmatrix}}
% complex numbers
\renewcommand{\Re}[1]{\operatorname{Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{\operatorname{Im}\left\{#1\right\}}
\newcommand{\conj}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
% probability and stat
\renewcommand{\P}[1]{\operatorname{\mathbb{P}}\left(#1\right)}
\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\dif}{\operatorname{d}}
\newcommand{\var}{\operatorname{var}}

% calculus
\renewcommand{\d}[1]{\,\mathrm{d}#1}

% constants (written in roman, if wanted)
%\newcommand{\e}{\mathrm{e}}
\renewcommand{\j}{\mathrm{j}}




\newcommand{\mb}{\bm}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\bb}{\mathbb}
\newcommand{\mrm}{\mathrm}
\newcommand{\mtt}{\mathtt}
\def \vecword  {\operatorname*{vec}}
% linear algebra
% 	vector notation
\newcommand{\vct}[1]{\boldsymbol{#1}}
%   matrices
\newcommand{\mtx}[1]{\boldsymbol{#1}}
%   block vector
\newcommand{\bvct}[1]{\mathbf{#1}}
%   block matrix
\newcommand{\bmtx}[1]{\mathbf{#1}}
%	inner products
\newcommand{\inner}[1]{\left<#1\right>}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
% 	transpose, Hermitian, pseudo-inverse
\renewcommand{\H}{\mathrm{H}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\pinv}{\dagger}
%	fundamental subspaces
\newcommand{\Null}{\operatorname{Null}}
\newcommand{\Range}{\operatorname{Range}}
\newcommand{\Span}{\operatorname{Span}}
%	operators
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\toep}{\operatorname{Toep}}
\newcommand{\SDP}{\operatorname{SDP}}
\newcommand{\PSD}{\operatorname{PSD}}
\newcommand{\far}{\operatorname{far}}
\newcommand{\near}{\operatorname{near}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Sign}{\operatorname{Sgn}}
\newcommand{\dist}{\operatorname{dist}}
\def \lg        {\langle}
\def \rg        {\rangle}
\def \vec       {\operatorname*{vec}}
%
\newcommand{\dimension}{\operatorname{dim}}

% sets and topology
\newcommand{\set}[1]{\mathbb{#1}}
\newcommand{\closure}{\operatorname{cl}}	% closure
\newcommand{\interior}{\operatorname{int}}
\newcommand{\boundary}{\operatorname{bd}}
\newcommand{\diameter}{\operatorname{diam}}

% functional analysis
\newcommand{\domain}{\operatorname{dom}}
\newcommand{\epigraph}{\operatorname{epi}}
\newcommand{\hypograph}{\operatorname{hypo}}
\newcommand{\linop}[1]{\mathscr{#1}}	% general linear operator

% optimization
\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\DeclareMathOperator*{\argmin}{\text{arg~min}}
\DeclareMathOperator*{\argmax}{\text{arg~max}}
\def \st {\operatorname*{s.t.\ }}
% other
%\newcommand{\sgn}{\text{sgn}}
\newcommand{\sinc}{\text{sinc}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\eps}{\epsilon}


\newcommand{\wh}{\widehat}
\newcommand{\wc}{\widecheck}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}


\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\nrm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bracket}[1]{\left( #1 \right)}
\newcommand{\parans}[1]{\left(#1\right)}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right)}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}
\newcommand{\iter}[1]{^{(#1)}}


\newcommand{\js}[1]{{\color{Mahogany} [\noindent JS: #1]}}

%--------------------------------------------------------------------------
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\hypersetup{
    colorlinks=true,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}

 \newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
 \newcommand{ \brac }[1]{\left[ #1 \right]}
% \newcommand{ \paren }[1]{ \left( #1 \right) }

\newcommand{\NC}{$\mc {NC}$}

\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vi}{\vct{i}}
\newcommand{\vj}{\vct{j}}
\newcommand{\vk}{\vct{k}}
\newcommand{\vl}{\vct{l}}
\newcommand{\vm}{\vct{m}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vo}{\vct{o}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
%
\newcommand{\valpha}{\vct{\alpha}}
\newcommand{\vbeta}{\vct{\beta}}
\newcommand{\vtheta}{\vct{\theta}}
\newcommand{\vepsilon}{\vct{\epsilon}}
\newcommand{\veps}{\vct{\epsilon}}
\newcommand{\vvarepsilon}{\vct{\varepsilon}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vnu}{\vct{\nu}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\vdelta}{\vct{\delta}}
\newcommand{\veta}{\vct{\eta}}
\newcommand{\vxi}{\vct{\xi}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vrho}{\vct{\rho}}
%
\newcommand{\vzero}{\vct{0}}
\newcommand{\vone}{\vct{1}}


\newcommand{\mA}{\mtx{A}}
\newcommand{\mB}{\mtx{B}}
\newcommand{\mC}{\mtx{C}}
\newcommand{\mD}{\mtx{D}}
\newcommand{\mE}{\mtx{E}}
\newcommand{\mF}{\mtx{F}}
\newcommand{\mG}{\mtx{G}}
\newcommand{\mH}{\mtx{H}}
\newcommand{\mJ}{\mtx{J}}
\newcommand{\mK}{\mtx{K}}
\newcommand{\mL}{\mtx{L}}
\newcommand{\mM}{\mtx{M}}
\newcommand{\mN}{\mtx{N}}
\newcommand{\mO}{\mtx{O}}
\newcommand{\mP}{\mtx{P}}
\newcommand{\mQ}{\mtx{Q}}
\newcommand{\mR}{\mtx{R}}
\newcommand{\mS}{\mtx{S}}
\newcommand{\mT}{\mtx{T}}
\newcommand{\mU}{\mtx{U}}
\newcommand{\mV}{\mtx{V}}
\newcommand{\mW}{\mtx{W}}
\newcommand{\mX}{\mtx{X}}
\newcommand{\mY}{\mtx{Y}}
\newcommand{\mZ}{\mtx{Z}}
%
\newcommand{\mGamma}{\mtx{\Gamma}}
\newcommand{\mDelta}{\mtx{\Delta}}
\newcommand{\mLambda}{\mtx{\Lambda}}
\newcommand{\mOmega}{\mtx{\Omega}}
\newcommand{\mPhi}{\mtx{\Phi}}
\newcommand{\mPsi}{\mtx{\Psi}}
\newcommand{\mSigma}{\mtx{\Sigma}}
\newcommand{\mTheta}{\mtx{\Theta}}
\newcommand{\mUpsilon}{\mtx{\Upsilon}}
%
\newcommand{\mId}{\bmtx{I}}
\newcommand{\mEx}{{\bf J}}
\newcommand{\mzero}{{\bf 0}}
\newcommand{\mone}{{\bf 1}}
%
\newcommand{\bva}{\bvct{a}}
\newcommand{\bvh}{\bvct{h}}
\newcommand{\bvw}{\bvct{w}}
\newcommand{\bvx}{\bvct{x}}
\newcommand{\bvy}{\bvct{y}}


\newcommand{\bmM}{\bmtx{M}}
\newcommand{\bmH}{\bmtx{H}}
\newcommand{\bmX}{\bmtx{X}}


\newcommand{\setA}{\set{A}}
\newcommand{\setB}{\set{B}}
\newcommand{\setC}{\set{C}}
\newcommand{\setD}{\set{D}}
\newcommand{\setE}{\set{E}}
\newcommand{\setF}{\set{F}}
\newcommand{\setG}{\set{G}}
\newcommand{\setH}{\set{H}}
\newcommand{\setI}{\set{I}}
\newcommand{\setJ}{\set{J}}
\newcommand{\setK}{\set{K}}
\newcommand{\setL}{\set{L}}
\newcommand{\setM}{\set{M}}
\newcommand{\setN}{\set{N}}
\newcommand{\setO}{\set{O}}
\newcommand{\setP}{\set{P}}
\newcommand{\setQ}{\set{Q}}
\newcommand{\setR}{\set{R}}
\newcommand{\setS}{\set{S}}
\newcommand{\setT}{\set{T}}
\newcommand{\setU}{\set{U}}
\newcommand{\setV}{\set{V}}
\newcommand{\setW}{\set{W}}
\newcommand{\setX}{\set{X}}
\newcommand{\setY}{\set{Y}}
\newcommand{\setZ}{\set{Z}}

\renewcommand{\ss}{{\vspace*{-1mm}}}

\setcounter{MaxMatrixCols}{20}

%\pagestyle{plain}

\graphicspath{{./figs/}}

\newlength{\imgwidth}
\setlength{\imgwidth}{3.125in}

\newcommand{\QW}[1]{\textcolor{red}{\bf [{\em QW:} #1]}}
\newcommand{\note}[1]{\textcolor{blue}{\bf [{\em Note:} #1]}}
\newcommand{\revise}[1]{\textcolor{blue}{#1}}
\newcommand{\edit}[1]{\textcolor{blue}{#1}}

\newboolean{twoColVersion}
\setboolean{twoColVersion}{false}
\newcommand{\twoCol}[2]{\ifthenelse{\boolean{twoColVersion}} {#1} {#2} }


\newcommand{\Poff}{\mathcal{P}_{\textup{off}}}
\newcommand{\Pon}{\mathcal{P}_{\textup{diag}}}

\newcommand{\cy}[1]{\textcolor{red}{\bf [{\em Can:} #1]}}
\newcommand{\qq}[1]{\textcolor{blue}{\bf [{\em Qing:} #1]}}
\newcommand{\pw}[1]{\textcolor{red}{\bf [{\em Peng:} #1]}}
\newcommand{\zz}[1]{\textcolor{blue}{ [{\em Zhihui:} #1]}}
\newcommand{\vvh}[1]{\textcolor{purple}{\bf [{\em WH:} #1]}}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}


%\newcommand{\calL}{\mathcal{L}}
\newcommand{\act}{\sigma}
\newcommand{\PrecAt}{\mathtt{Prec}\mbox{@}}

\newcommand{\pow}{\mathcal{P}}

% macros.tex
% useful macros (shortcuts) to save typing; add more as needed!

\newtheorem{proposition}{\bf{Proposition}}
%\newtheorem{remark}{\bf{Remark}}
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}

% now define useful macros

\long\def\comment#1{}
\newcommand{\fref}[1] {Fig.~\ref{#1}\xspace}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\Expi}[1]{\mathrm{e}^{\imath #1}}
\newcommand{\xtrue}{\xmath{\x_{\text{true}}}}
\newcommand{\cdft}{\xmath{c_{\text{dft}}}}
%\newcommand{\argmin}{\operatorname{argmin}\ }
%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\tr}{\operatorname{tr}}
%\newcommand{\st}{\operatorname{s.t.}}
\newcommand{\range}{\operatorname{Range}}
%\newcommand{\rank}{\operatorname{rank}}
\renewcommand{\dim}{\operatorname{dim}}
\newcommand{\pri}{\text{pri}}
\newcommand{\dual}{\text{dual}}
\newcommand{\etal}{\textit{et al. }}
%\newcommand{\bmat}[1] {\begin{bmatrix} #1 \end{bmatrix}} % best arrays ever

\newcommand{\xmath}[1] {\ensuremath{#1}\xspace}
\newcommand{\blmath}[1] {\xmath{\bm{#1}}}
\newcommand{\A}{\blmath{A}}
\newcommand{\B}{\blmath{B}}
%\newcommand{\C}{\blmath{C}}
\newcommand{\D}{\blmath{D}}
%\newcommand{\E}{\blmath{E}}
\newcommand{\F}{\blmath{F}}
\newcommand{\I}{\blmath{I}}
%\newcommand{\R}{\blmath{R}}
%\newcommand{\T}{\blmath{T}}
\newcommand{\U}{\blmath{U}}
\newcommand{\V}{\blmath{V}}
\newcommand{\W}{\blmath{W}}
\newcommand{\X}{\blmath{X}}
\newcommand{\Y}{\blmath{Y}}
%\newcommand{\Z}{\blmath{Z}}

\newcommand{\x}{\blmath{x}}
\newcommand{\s}{\blmath{s}}
\newcommand{\y}{\blmath{y}}
\newcommand{\z}{\blmath{z}}
\newcommand{\1}{\blmath{1}} 
\newcommand{\0}{\blmath{0}} 
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\ie}{\text{i.e.}}
\newcommand{\eg}{\text{e.g.}}

\newcommand{\bLam}{\blmath{\Lambda}}


\let\originalu\u
\let\originalv\v

\newcommand{\bi} {\xmath{b_i}}
\newcommand{\hi} {\xmath{h_i}}
\newcommand{\dhi} {\xmath{\dot h_i}}
\newcommand{\ddhi} {\xmath{\ddot h_i}}
\newcommand{\ti} {\xmath{t_i}}
\newcommand{\ui} {\xmath{u_i}}
%\newcommand{\vi} {\xmath{v_i}}
\newcommand{\yi} {\xmath{y_i}}

\newcommand{\defequ} {\triangleq}
\newcommand{\sumi} {\xmath{\sum_i \; }}
\newcommand{\Wmax}{\xmath{\W_{\max}}}
\newcommand{\Wimp}{\blmath{W}_{\mathrm{imp}}}
%\newcommand{\real}[1] {\mathrm{real}\!\left\{#1\right\}}
%\newcommand{\sign}[1] {\mathrm{sign}\!\left(#1\right)}
%\newcommand{\abs}[1] {\left| #1 \right|}
\newcommand{\absb}[1] {\big| #1 \big|}
\newcommand{\Half} {\frac{1}{2}}

\newcommand{\notezl}[1] {\textcolor{red}{ZL: #1}}

%\newcommand{\reals} {\xmath{\mathbb{R}}}
%\newcommand{\complex} {\xmath{\mathbb{C}}}
\newcommand{\RM} {\xmath{\reals^M}}
\newcommand{\CN} {\xmath{\complex^N}}
\newcommand{\baih} {\xmath{\ba_i'}}
\newcommand{\psii} {\xmath{\psi_i}}
\newcommand{\bpsi} {\blmath{\psi}}

\newcommand{\Ah} {\xmath{\A'}}

\newcommand{\xk} {\xmath{\blmath{x}_k}}
\newcommand{\xkk} {\xmath{\blmath{x}_{k+1}}}
\newcommand{\zkk} {\xmath{\blmath{z}_{k+1}}}
\newcommand{\dk} {\xmath{\blmath{d}_k}}
%\newcommand{\vk} {\xmath{\blmath{v}_k}}
\newcommand{\vkk} {\xmath{\blmath{v}_{k+1}}}
\renewcommand{\u} {\blmath{u}}
\renewcommand{\v} {\blmath{v}}

\newcommand{\figref}[2] {Fig.~\ref{#1}}
\newcommand{\figcap}[3] { % file width caption
\begin{figure}
    \centering
    \includegraphics[width=#2\linewidth]{fig/#1}
    \caption{#3}
    \label{fig:#1}
\end{figure}
}

% KL below here

%\newcommand{\qed}{\hfill\rule{2mm}{2mm}}
\newcommand{\svskip}{\vspace{1.75mm}}
\newcommand{\mvskip}{\vspace{.25in}}
\newcommand{\lvskip}{\vspace{.5in}}
\def\E{\mathop{\rm E\,\!}\nolimits}
\def\Var{\mathop{\rm Var}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\den{\mathop{\rm den}\nolimits}
\def\midd{\mathop{\,|\,}\nolimits}
\def\sgn{\mathop{\rm sgn}\nolimits}
\def\vec{\mathop{\rm vec}\nolimits}
\def\sinc{\mathop{\rm sinc}\nolimits}
\def\curl{\mathop{\rm curl}\nolimits}
\def\div{\mathop{\rm div}\nolimits}
\def\tr{\mathop{\rm tr}\nolimits}
\def\len{\mathop{\rm len}\nolimits}
%\def\diag{\mathop{\rm diag}\nolimits}
\def\dist{\mathop{\rm dist}\nolimits}
\def\amp{\mathop{\;\:}\nolimits}

\newcommand{\ba}{\boldsymbol{a}}

\newcommand{\bbb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
%\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bl}{\boldsymbol{l}}
%\newcommand{\bm}{\boldsymbol{m}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bo}{\boldsymbol{o}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bN}{\boldsymbol{N}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}


\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bleta}{\boldsymbol{\eta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btheta}{\xmath{\bm{\theta}}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\def\b{{\blmath b}} 
\def\L{{\cal L}}
\newcommand{\paren}[1]{\left( #1 \right)}
\long\def\red#1{\bgroup\color{red}#1\egroup}

\newcommand{\of}[1]{\!\paren{#1}}
\newcommand{\dH} {\xmath{\dot{H}}}
\newcommand{\Xs} {\xmath{\mathcal{X}_s}}
\newcommand{\Lip} {\xmath{\mathcal{L}}}
\newcommand{\copt}{\xmath{c_{\mathrm{opt}}}}
\newcommand{\cimp}{\xmath{c_{\text{imp}}}}
\newcommand{\todo}[1]{\textbf{Todo: #1}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\ith}{i^{\mathrm{th}}}


\definecolor{mich-blue}{HTML}{0027CC}
\definecolor{mich-blue-high}{HTML}{0027CC}
%\definecolor{mich-blue}{HTML}{00274C}
%\definecolor{mich-blue-high}{HTML}{00408C}
\definecolor{red-high}{HTML}{CA2020}
\definecolor{green-high}{HTML}{20A520}
\definecolor{mich-maize}{HTML}{FFCB05}
\definecolor{law-stone}{HTML}{655A52}
\definecolor{burton-beige}{HTML}{9B9A9D}
\definecolor{arch-ivy}{HTML}{7E732F}

\newcommand{\highlight}[1]{\textcolor{mich-blue-high}{#1}} 
\newcommand{\highlightred}[1]{\textcolor{red-high}{#1}} 
\newcommand{\highlightgreen}[1]{\textcolor{green-high}{#1}} \colorlet{color1}{gray!15}
\newcommand{\hlnew}[1] {\highlight{\colorbox{color1}{#1}}}
\newcommand{\xtz} {\xmath{\tilde{\blmath{x}}_0}}
\newcommand{\fF}{\xmath{\mathbb{F}}}
\newcommand{\eE}{\xmath{\mathbb{E}}}
\newcommand{\FN}{\xmath{\fF^N}}
\newcommand{\FNN}{\xmath{\fF^{N\times N}}}
\newcommand{\subdot} {_{\bm{\cdot}}}

==> section/conclusion.tex <==

\section{Discussion and Future Directions}\label{sec:conclusion}

In this work, we conducted an in-depth study of an important but largely overlooked phenomenon in diffusion models, for which we term it as ``consistent model reproducibility''. This study raises numerous compelling questions that are worth further exploration, which we discuss in the folllowing

\paragraph{Practical applications.} One such question is the tangible practical benefits of model reproducibility in diffusion models compared to other types of generative models. One major insight gained from this study is that the mapping from the noise space to the image space is a unique one-to-one mapping, regardless of network architectures or training procedures. This observation implies that the noise space contains valuable information that can be utilized for controlled data generative processes using diffusion models. For instance, in text-driven image generation tasks, a deeper understanding of this mapping could facilitate content generation, by leveraging the same text embeddings while varying noise inputs, there are potential applications including adversarial attacks \citep{zou2023universal} (noise that will always map to adversarial generation), robust defense \citep{zhu2023promptbench} (noise that robust to adversarial text input), and copyright protection \citep{somepalli2023understanding, somepalli2023diffusion} (noise that not memorize data). Moreover, in the context of solving inverse problems, a definitive answer to this question could guide us to select the input noise for reducing the uncertainty and variance in our signal reconstruction  ~\citep{langevin,chung2022score-MRI,luo2023bayesian}. 

\paragraph{Theoretical understandings.} Moreover, the strong connection between model reproducibility and generalizability opens an enticing theoretical question for further study. While the phenomenon of ``consistent model reproducibility'' in the memorization regime has been comprehensively explained in this work, the understanding of this phenomenon in the generalization regime, particularly the identifiable mapping between the noise space and image space, remains an unresolved but valuable question. Recently, the work \cite{yi2023generalization} has developed a framework for analyzing the generalizability of diffusion models, which might offer valuable insights into the reproducibility analysis due to the strong connection between reproducibility and generalizability.

On the other hand, numerous recent studies \citep{shi2023diffusion, de2021diffusion, luo2023image, delbracio2023inversion, liu20232, khrulkov2022understanding} have explored the connection between diffusion models and the Schrödinger bridge, treating the encoding process from the image space to the noise space as an optimal transport problem. The identifiable relationship could be potentially derived as the solution to the optimal transport problem.

%\begin{itemize}
 %   \item \textbf{Uniquely Identifiable Encoding.} \cite{song2020score} have stated that the diffusion model is a uniquely identifiable encoding. Nevertheless, their research primarily relied on some preliminary experiments as evidence for this claim and also lacked a comprehensive theoretical investigation to elucidate this mapping. Notably, the exploration of uniquely identifiable encoding has been extensively examined in various other domains of machine learning (i.e. ICA \citep{hyvarinen2016unsupervised, hyvarinen2017nonlinear, hyvarinen2019nonlinear}, VAE given a factorized prior distribution \cite{khemakhem2020variational}, conditional energy-based models \cite{khemakhem2020ice}, representation learning \cite{roeder2021linear}) Hence, an in-depth theoretical analysis of uniquely identifiable encoding in these areas might offer insights into the analysis of diffusion models.
 %   \item \textbf{Schrödinger Bridge and Optimal Transport}. 
 %   \item \textbf{Generalizability of Diffusion Model}. \cite{yi2023generalization} has developed a framework for analyzing the generalizability of diffusion models, which might offer valuable insights into the reproducibility analysis because of the strong connection between reproducibility and generalizability.
%\end{itemize}




%In this study, we provided an in-depth study of an intriguing phenomenon in diffusion models that has been largely overlooked, which we term ``consistent model reproducibility''. Our work opens many interesting questions worth further investigation. For example, the practical benefits of model reproducibility of diffusion models over other types of generative models worth further investigation. Moreover, how to theoretically understand the relationship between model reproducbility and generalizability in the generalization regime is a very interesting question.



%Furthermore, our investigation has brought to light that this remarkable model reproducibility occurs in two specific training scenarios: (i) ``memorization regime,'' (ii) ``generalization regime.'' Our analysis also provides theoretical support for model reproducibility during the ``memorization regime.'' Additionally, our research has demonstrated that this valuable attribute extends to variants of diffusion models, encompassing conditional diffusion models, diffusion models for inverse problems, and fine-tuned diffusion models.


==> section/intro.tex <==


\section{Introduction}

 Recently, diffusion models have emerged as a powerful new family of deep generative models with remarkable performance in many applications, including image generation \citep{ho2020denoising, song2020score, rombach2022high}
 %~\cite{ddpm, song2021scorebased, ddim, stablediffusion}
 , image-to-image translation \citep{su2022dual,saharia2022palette, zhao2022egsde}, text-to-image synthesis \citep{rombach2022high, ramesh2021zero, nichol2021glide}, and solving inverse problem solving \citep{chung2022improving, song2022pseudoinverse, chung2022diffusion,song2023solving}.
 %~\cite{chung2022mcg, song2023Pseudoinverse, dps}
 %, and scientific discovery \citep{song2021solving, langevin, chung2022score-MRI, aali2023solving-noisy, kazerouni2022diffusion-medimage,zhang2023molecule, wu2022diffusion-molecule, xu2023geometric-molecule, luo2021predicting-molecule, xu2022geodiff-molecule, peng2023moldiff}. 
 These models learn an unknown data distribution generated from the Gaussian noise distribution through a process that imitates the non-equilibrium thermodynamic diffusion process \citep{ho2020denoising, song2020score}. In the forward diffusion process, the noise is continuously injected into training samples; while in the reverse diffusion process, a model is learned to remove the noise from noisy samples parametrized by a noise-predictor neural network. Then guided by the trained model, new samples (e.g., images) from the target data distribution can be generated by transforming random noise instances through step-by-step denoising following the reverse diffusion process. Despite the remarkable data generation capabilities demonstrated by diffusion models, the fundamental mechanisms driving their performance are largely under-explored.

%

% \begin{figure}
%      \centering
%      \begin{subfigure}[t]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/unconditional_sample/DDPMv4.png}
%          \caption{DDPMv4}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.32\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/unconditional_sample/ct.png}
%          \caption{CT}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.32\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/unconditional_sample/UViT.png}
%          \caption{U-ViT}
%      \end{subfigure}
%      \caption{\textbf{Unconditional diffusion model samples visualization.} We utilized denoising diffusion probabilistic models (DDPM) \cite{ho2020denoising, song2020denoising}, consistency model (CT) \cite{song2023consistency}, U-ViT \cite{bao2023all} trained on CIFAR-10 \cite{krizhevsky2009learning} dataset released by the author. Samples in the corresponding row and column are generated from the same initial noise with a deterministic ODE sampler. More details are shown in Table \ref{tab:unconditional_setting} in Appendix \ref{append:unconditional}.}
%      \label{fig:unconditional_sample}
% \end{figure}

% \begin{figure}
%      \centering
%      \begin{subfigure}[t]{1.0\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/unconditional_sample/uncon_3_figs.pdf}
%          \caption{DDPMv4}
%      \end{subfigure}
%      \caption{\textbf{Unconditional diffusion model samples visualization.} We utilized denoising diffusion probabilistic models (DDPM) \cite{ho2020denoising, song2020denoising}, consistency model (CT) \cite{song2023consistency}, U-ViT \cite{bao2023all} trained on CIFAR-10 \cite{krizhevsky2009learning} dataset released by the author. Samples in the corresponding row and column are generated from the same initial noise with a deterministic ODE sampler. More details are shown in Table \ref{tab:unconditional_setting} in Appendix \ref{append:unconditional}.}
%      \label{fig:unconditional_sample}
% \end{figure}





In this work, to better understand diffusion models, we study the following fundamental question:
\begin{tcolorbox}
\begin{center}
   \textbf{Q1:} \emph{Starting from the \textbf{same noise input}, how are the generated data samples from various diffusion models related to each other?}
\end{center}
\end{tcolorbox}
% \qq{discuss the implications of our results in this paragraph, I will leave this to Liyue a bit} 

 

A deeper understanding of this question has the potential to yield more interpretable and controlled data generative processes of using the diffusion models in many application disciplines~\citep{zhang2023adding, epstein2023diffusion}. For example, in the text-driven image generation, insights into this question could help to guide the content generation (e.g., adversial attacking \citep{zou2023universal}, robust defending \citep{zhu2023promptbench}, copyright protection \citep{somepalli2023understanding, somepalli2023diffusion}) using the same text embedding but varying noise inputs.
In solving inverse problems, an answer to this question will guide us to select the input noise for reducing the uncertainty and variance in our signal reconstruction ~\citep{langevin,chung2022score-MRI,luo2023bayesian}. Theoretically, understanding the question will shed light on how the mapping function is learned and constructed between the noise and data distributions, which is crucial for understanding the generation process through the distribution transformation or identifiable encoding~\citep{roeder2021linear, khemakhem2020variational, khemakhem2020ice}. 

%what results are expected given the same text input while different noise input; how this behavior can perform with different diffusion models. 



%In the constrained generation process such as using diffusion models for solving inverse problems, given the same observation constrains, different noise input will yield different output with uncertainty and variance~\citep{langevin,chung2022score-MRI,luo2023bayesian}. How shall we select the input noise to the constrained generation process has become an unsolved question in all these existing works using diffusion models as generative priors~\citep{langevin,chung2022score-MRI,song2021solving}.
%the answer to this question discloses an essential and intrinsic property of diffusion models that More importantly, leveraging such a unique property of diffusion models can particularly benefit the conditional or constrained generation process.  Therefore, the investigation in this study will potentially benefit and advance the controllable data generation based on diffusion models 
%How does the property of unique identifiable encoding benefit the diffusion model? To begin with, this is a large step toward the interpretability of the diffusion model; Secondly, it gives a potential for controllable generation; Beyonds 

\begin{figure}[t]
     \centering
     \includegraphics[width=1.\textwidth]{figure/unconditional_sample/uncon_3_figs.pdf}
     \caption{\textbf{Unconditional diffusion model samples visualization.} We utilized denoising diffusion probabilistic models (DDPM) \citep{ho2020denoising, song2020denoising}, consistency model (CT) \citep{song2023consistency}, U-ViT \citep{bao2023all} trained on CIFAR-10 \citep{krizhevsky2009learning} dataset released by the author. Samples in the corresponding row and column are generated from the same initial noise with a deterministic ODE sampler. More details are shown in Table \ref{appendtab:unconditional_setting} in Appendix \ref{append:unconditional}.}
     \label{fig:unconditional_sample}
\end{figure}

In this work, we provide an in-depth study of the question and uncover an intriguing and prevalent phenomenon within the diffusion model that sets it apart from most other generative models. We term this phenomenon as ``\emph{consistent model reproducibility}''. More precisely, as illustrated in \Cref{fig:unconditional_sample}, when different diffusion models are trained on the same dataset and generate new samples through a deterministic ODE sampler from the same noises, we find that \emph{all diffusion models generate nearly identical images, which is irrespective of network architectures, training and sampling procedures, and perturbation kernels.}

The consistent model reproducibility we identified for diffusion models is similar to the notion of unique identifiable encoding for deep latent-variable models, which is the property that the learned input-embedding is reproducible towards an identifiable mapping, regardless of different weight initialization or optimization procedures \citep{roeder2021linear}. The property was first proved by \cite{hyvarinen2016unsupervised, hyvarinen2017nonlinear, hyvarinen2019nonlinear} on the analysis of Independent Component Analysis (ICA) and extended to deep latent-variable models. Recently, \cite{khemakhem2020variational} demonstrated the identifiability of Variational Autoencoder (VAE) based on conditionally factorial priors distribution over the latent variables, \cite{khemakhem2020ice} consider the identifiability theory for conditional energy-based models and \cite{roeder2021linear} proved a linear identifiability on representation learning. In comparison, the consistent model reproducibility of diffusion models studied in this work implies that we are learning a unique encoding between the noise space and the image space. 



 %only on unconditional diffusion models and the results are 
 
 %In contrast, we provide an in-depth study of model reproducibility for many variants of diffusion models, identifying a strong relationship between model reproducibility and generalizability.


More interestingly, as illustrated in \Cref{fig:theoretical_analysis}, we find that the consistent model reproducibility of diffusion models emerges in two distinct regimes: (\emph{i}) "\emph{memorization regime}" where the model has large capacity of memorizing the training data but no ability to generate new samples, and (\emph{ii}) "\emph{generalization regime}" where the model regain the consistent model reproducibility and can also produce new data. In this work, we provide theoretical justification for the memorization regime. Moreover, the simultaneous occurrence of reproducibility and generalizability in the model generalization regime presents an interesting open question that is worth of future study.
%\sly{give any hypothesis here?}

%More interestingly, we identify that the consistent model reproducibility of diffusion models emerges in two distinct regimes of training:
 %(a) ``\emph{data memorization regime}'' and (b) \emph{model generalization regime}, where both regimes have strong correlation with the model's generalizability. First, the ``data memorization regime'' is a regime where the model is overparameterized and trained on data of small size. In this regime, although the model possesses the power of reproducibility (see \Cref{xx} xx), the generated data is simply a memoerization of training data and the model does not have the full ability of generating new samples (see \Cref{xx}). Although this is a regime of less interest in practice, we rigorously characterized the global solution in theory, and demonstrated that the diffusion models will reproduce the theoretical solution. Second, the ``model generalization regime'' is the other regime that the model is trained on large dataset and possess the power of generating new data (see \Cref{xx}). Surprisingly, when the training data size increases, the model regains reproducibility (see \Cref{xx}) while it is able to generate new samples. This is the regime where the diffusion models are trained in practice, and the cooccurence of model's reproducibility and generalizability is an intriguing phenemonon that is not fully understood. Our work opens an interesting theoretical question worth further investigation.

%The second regime is called ``\textbf{model generalizability regime}''. This is the regime where the diffusion model gains model 

% the model reproducibility emerges when trained on small training data, and gradually disappears when the training data size becomes large. ， 

  \renewcommand\thempfootnote{\arabic{mpfootnote}}
\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figure/analysis/comparison_3_curves_v5.png}
         \caption{Reproducibilty}
         \label{fig:reproducibility}
     \end{subfigure}
     \hspace{5mm}
     % \hfill
     \begin{subfigure}[t]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figure/analysis/comparion_generaliztion_v5.png}
         \caption{Generalizability}
         \label{fig:regime}
     \end{subfigure}
     \hfill
     \caption{\textbf{``Memorization'' and ``Generalization'' regimes for unconditional diffusion models.} We utilize DDPMv4 and train them on the CIFAR-10 dataset, adjusting both the model's size and the size of the training dataset. In terms of model size, we experiment with UNet-64, UNet-128, and UNet-256, where, for instance, UNet-64 indicates a UNet structure with an embedding dimension of 64. As for the dataset size, we select images from the CIFAR dataset, ranging from $2^6$ to $2^{15}$. Under each dataset size, different models are trained from the same subset of images. The figure on the left displays the reproducibility score as we compare various models across different dataset sizes, while the figure on the right illustrates the generalizability score of the models as the dataset size changes.
  %   \sly{shall this figure be shown earlier?}
     }    
   \label{fig:theoretical_analysis}
\end{figure}


Finally, we show that the consistent model reproducibility could be generalized to many other variants of diffusion model settings: conditional diffusion models, diffusion models for solving inverse problem, and fine-tuning diffusion models. 
Regarding conditional diffusion models, the model reproducibility is not only evident among different conditional diffusion models, but also it manifests in a structured way when comparing conditional models to their unconditional counterparts. Concerning solving inverse problem by using diffusion models as generative priors, we observe that the model reproducibility is confined within models using the same type of network architectures (e.g., either U-Net based or transformer-based architecture). Finally, in the context of fine-tuning diffusion models, we show partial fine-tuning of pretrained models reduces reproducibility but improves generalizability in ``memorization regime'' when compared to training from scratch.

%reproducibility is not only observed within different conditional diffusion models but also manifests in a specific way when comparing unconditional and conditional diffusion models; 
% where the new data sample is generated with the data consistency constraint during inference time,
% specifically within the context of the diffusion model with soft data consistency \hjz{I am not sure about the name, Liyue}, 

% it is noteworthy that fine-tuning specific portions of the model may diminish the model reproducibility while enhancing generalizability, especially in scenarios with limited data, ``memorization regime''. %\qq{expand here for more details in this paragraph, Huijie}
%\qq{todo rephrase }





 
% Interestingly, as shown in Figure \Cref{fig:reproducibility_selected} we find this property is ubiquitous among different diffusion model architectures, with no need for any conditional prior, regardless of model architecture, diffusion model perturbation kernel, and many other training settings.

%It should noted that the phenomenon of consistent model reproducibility has been observed in the recent seminal work \cite{song2020score} and subsequent works \cite{xx}, however, the experimental investigation is only on unconditional diffusion models and is very preliminary.


%we systematically analyze the reproducibility of the unconditional diffusion model given different architectures, perturbation kernel, and many other training settings. In Section \ref{sec:reproducibility_more} we investigate this property in the conditional diffusion model, projection-based diffusion model, and diffusion model fintuning. In specific, for the conditional diffusion model we find it is not only reproducibility and there is a reproducible relationship with the unconditionaly diffusion model; for the projection-based diffusion model, we find the reproducibility in the gradient space of score function only holds for similar architecture. And for \hjz{conclusion for fintuning}. In Section \ref{sec:analysis}, we theoretically prove the identifiable encoding of the diffusion model and experimentally verify it in a special case. And we display a potential relationship between reproducibility and generalizability. 


\paragraph{Summary of Contributions.} In summary, we briefly highlight our contributions below:
\begin{itemize}[leftmargin=*]
  \item \textbf{Model reproducibility of unconditional diffusion models (\Cref{sec:uncond}).} We provide a systematic study of the of the unconditional diffusion model, regardless of the choices of network architectures, perturbation kernels, training and sampling settings.
     \item \textbf{Two regimes of model reproducibility (\Cref{sec:analysis}).} We find a strong correlation between reproducibility and generalizability for diffusion model. We provide a theoretical study for the memorization regime.
   \item \textbf{Model reproducibility of variants of diffusion models (\Cref{sec:reproducibility_more}).} We reveal the reproducibility in more various diffusion model settings, including conditional diffusion models, diffusion models for inverse problem solving, and fine-tuning diffusion models.
\end{itemize}
Finally, we conclude and discuss the implications of our results in \Cref{sec:conclusion}.
%The rest of the paper is organized as follows. In \Cref{sec:reproducibility_unconditional}, we study consistent model reproducibility for unconditional diffusion models. In \Cref{xx}, we extend our study to variants of other diffusion models. Finally, we conclude and discussion the implications of our results in \Cref{xx}.


%In this paper, we will systematically uncover the unique identifiable encoding property of the diffusion model. We demonstrate that for all the unconditional diffusion models we used in this paper, after training with the same dataset and using an ODE sampler, the same initial noise will generate almost the same result. Furthermore, we show that this property is also prevalent in many other diffusion model settings: conditional diffusion, projection-based diffusion model, and diffusion model fintuning. In addition, we also explicitly express the mathematical formulation of the unique identifiable encoding. Our experiments demonstrate that the diffusion model does converge to this theoretical solution in specific cases. However, in a more general setting, the diffusion model converges to another unique encoding but is far from our theoretical proof, which leaves an open question for future research.

%We demonstrate that for all the unconditional diffusion models we used in this paper, after training with the same dataset and using an ODE sampler, the same initial noise will generate almost the same result.





%Recently, the diffusion model gradually become one of the hottest topics for generative models and computer vision \cite{croitoru2023diffusion}. Originating from unconditional generation \cite{ho2020denoising, song2020score}, the diffusion model displays its versatility in its diversified application: Conditional Image Generation \cite{dhariwal2021diffusion, ho2022classifier}, Image-to-Image Translation \cite{su2022dual,saharia2022palette, zhao2022egsde}, Text-to-Image generation \cite{rombach2022high, ramesh2021zero, nichol2021glide}, inverse problem solving \cite{song2023solving,chung2022diffusion,song2021solving}, video generation \cite{ho2022imagen, harvey2022flexible}, and so on. While people are focusing on the amazing ability of the diffusion model on generation quality, we uncover another property that is omnipresent for the diffusion model, \textit{Unique identifiable encoding} \cite{song2020score}.















==> section/phenomenon.tex <==

\section{Study for Unconditional diffusion models}\label{sec:uncond}


%In this section, we initiate our study on unconditional diffusion models in \Cref{subsec:uncond-diffusion}, and study the relationship between model reproducibility and generalizability in \Cref{subsec:generalization}.

For unconditional diffusion models, new samples (e.g., images) are generated by transforming \emph{randomly sampled noise instances} through a reverse diffusion process guided by the trained model \citep{ho2020denoising, song2020score}. If we start from the \emph{same} noise input and use a deterministic ODE sampler, we observe that 
\begin{tcolorbox}
\begin{center}
   \textbf{C2:} \emph{Diffusion models consistently generate \textbf{nearly identical contents}, irrespective of network architectures, training and sampling procedures, and perturbation kernels.}
\end{center}
\end{tcolorbox}
%This seems to be obvious by examining the visualized samples generated by different diffusion models, as we shown in \Cref{fig:unconditional_sample} we visualize different samples generated from DDPM \cite{ho2020denoising}, Consistency Training (CT) \cite{song2023consistency}, and U-ViT \cite{bao2023all} starting from the same noise. Interestingly, for the same noise initialization, different diffusion models (i.e., DDPM \cite{ho2020denoising}, Consistency Training (CT) \cite{song2023consistency}, and U-ViT \cite{bao2023all}) generate nearly identical samples with very similar low-level color structures. \qq{we conducted on cifar10, but other papers xxxx}
This seems to be obvious by examining the visualized samples generated by different diffusion models in \Cref{fig:unconditional_sample} -- starting from the same noise input, different diffusion models (i.e., DDPM \citep{ho2020denoising}, Consistency Training (CT) \citep{song2023consistency}, and U-ViT \citep{bao2023all}) generate nearly identical samples with very similar low-level color structures. More recent seminal \citep{song2020score} has observed a similar phenomenon (see also subsequent works \citep{song2023consistency, karras2022elucidating}), but the study in \cite{song2020score} remains preliminary.  


\subsection{Evaluation Setup of Model Reproducibility}\label{subsec:uncond-diffusion}

While the findings in \Cref{fig:unconditional_sample} are intriguing, the basic visualization alone is not sufficient to fully justify our claim. For a more comprehensive study, we first introduce quantitative measures for model reproducibility and basic experimental setup.


\subsubsection{Quantitative Measures of Model Reproducibility} \label{sec:metric}
To study this phenomenon more quantitatively, we introduce the \textit{reproducibility (RP) score} to measure the similarity of image pair generated from two different :diffusion models starting from the same noise drawn i.i.d. from the standard Gaussian distribution. Specifically, we define
\begin{align*}
    \text{RP Score} \;:=\; \mathbb{P}\paren{\mathcal{M}_{\text{SSCD}}(\bm x_1, \bm x_2)>0.6},
\end{align*}
represents the \emph{probability} of a generated sample pair $(\bm x_1, \bm x_2)$ from two different diffusion models to have \emph{self-supervised copy detection} (SSCD) similarity $\mathcal{M}_{\text{SSCD}}$ larger than $0.6$ \citep{pizzi2022self, somepalli2023understanding} ($\mathcal{M}_{\text{SSCD}} > 0.6$ exhibits strong visual similarities). We sampled 10K noise to estimate the probability. 
%In our experiment, we measure this probability empirically based upon $10^4$ random noise samples drawn i.i.d. from the standard Gaussian distribution.
The SSCD similarity is first introduced in \cite{pizzi2022self} to measure the replication between image pair $(\bm x_1, \bm x_2)$, which is defined as the following: 
%\qq{make the math x italic}
\begin{align*}
    \mathcal{M}_{\text{SSCD}}(\bm x_1, \bm x_2) = \dfrac{\text{SSCD}(\bm x_1) \cdot \text{SSCD}(\bm x_2)}{||\text{SSCD}(\bm x_1)||_2 \cdot ||\text{SSCD}(\bm x_2)||_2}
\end{align*}
where $\text{SSCD}(\cdot)$ represents a neural descriptor for copy detection. 
%In our work, we use the \emph{Reproducibility Score} to measure the replication between two different diffusion models. 
%For evaluating the model reproducibility, we measure $\mathcal{I}_{\text{SSCD}}$ for each image pair generated from two different diffusion models starting from the same noise and count the reproducibility score for all image pairs.
%In \cite{somepalli2023understanding}, they count a visual replication of two models when $\text{SSCD}\geq 0.4$. Here, we use a larger threshold $\mathcal{I}_{\text{SSCD}}>0.6$. \qq{why we use a larger threshold?} \hjz{As shown in previous, for $\mathcal{I}_{\text{SSCD}} \geq$ 0.4, sometimes it means similar object but in different color, so we want to make the metric more strict to identical image}

In addition, we also use the \emph{mean-absolute-error (MAE) score} to measure the reproducibility, $\text{MAE Score} := \mathbb{P}\paren{\text{MAE}(\bm x_1, \bm x_2)<15.0}$ , similar setting with the RP score. $\text{MAE}(\cdot)$ is the operator that measures the mean absolute different of image pairs in pixel value space ([0, 255]). The quantitative results for selected diffusion model architectures are shown in Figure \ref{fig:reproducibility_selected}. %\qq{state MAE score first, then MAE}

\subsubsection{Experimental Setup for Evaluation} In this work, we conduct a comprehensive study of model reproducibility based upon different network architectures, model perturbation kernels, and training and sampling processes:  
\begin{itemize}
    \item \textbf{Network architectures.}
We evaluate for both UNet \citep{ronneberger2015u} based architecture: DDPM \citep{ho2020denoising}, DDPM++ \citep{song2020score}, Multistage \citep{multistage}, EDM \citep{karras2022elucidating}, Consistency Training (CT) and Distillation (CD) \citep{song2023consistency};  Transformer \citep{vaswani2017attention} based architecture: DiT \citep{peebles2022scalable} and U-ViT \citep{bao2023all}.
\item \textbf{Training Process.} We also considered discrete \citep{ho2020denoising} or continuous \citep{song2020score} settings, estimating noise $\epsilon$ or original image $\bm x_0$, training from scratch or distillation \citep{salimans2022progressive, song2023consistency} for the diffusion model.
\item \textbf{Perturbation Kernels.} For noise perturbation stochastic differential equations, we use Variance Preserving (VP) \citep{ho2020denoising}, Variance Exploding (VE), sub Variance Preserving (sub-VP) \citep{song2020score}. All the models are trained with the CIFAR-10 dataset \citep{krizhevsky2009learning} until convergence.\footnote{Here, convergence means achieving the lowest Fréchet inception distance (FID) \cite{heusel2017gans}.} 
\item  \textbf{Sampling Process.} For sampling, we only used the \emph{deterministic} sampler, such as DPM-Solver \citep{lu2022dpm}, Heun-Solver \citep{karras2022elucidating}, DDIM \citep{song2020denoising} etc. We use the deterministic sampler instead of the stochastic sampler, because randomness introduced by stochastic samplers will break the model reproducibility.
\end{itemize}
% \qq{check below}
In the process of sampling, it’s important to not that we exclusively use deterministic samplers for two main reasons. First, stochastic samplers (e.g. \cite{ho2020denoising}) introduce random noise at every time step, leading to a lack of model reproducibility. Second, many recent advanced samplers, such as those proposed in \citep{song2020denoising, lu2022dpm, karras2022elucidating, zhang2022fast} are deterministic samplers. These deterministic samplers lead to fast sampling speed, and have been successfully applied not only to unconditional diffusion models but also to diffusion models for solving inverse problems \citep{song2023solving}, large text-to-image diffusion model \citep{rombach2022high} and so on.
%\qq{should this be sampling process?} \textbf{(a) Model Architectures.} 
 
% \cite{somepalli2023understanding} using self-supervised copy detection (SSCD) metric  to measure the replication between generated images from the diffusion model and the original dataset. Inspired by their setting, we design the \textit{reproducibility score} to measure the replication between two different diffusion models. We randomly sampled 10K noise from the Gaussian distribution and used the same noise for all diffusion models to generate images. For each two diffusion models, we measured the SSCD distance for all image pairs generated from the same noise. Usually, SSCD score above $> 0.4$ reflects a visual replication \cite{somepalli2023understanding}. For \textit{reproducibility score}, it represents the percentage of generation pairs having SSCD similarity $> 0.6$ between two diffusion models. 

\subsection{Model Reproducibility of Unconditional Diffusion Models}\label{subsec:uncond-diffusion-modelreproducibility}

%\subsection{Samples visualization}
%More than quantitative analysis, we present some generated samples from the same initial noise shown in Figure \ref{fig:unconditional_sample} from DDPMv4, CT, and UViT. More results are shown in Appendix \ref{append:more_results}. In general, most of the generated samples look exactly the same. Even samples that look not exactly the same, share very similar low-level color structures (for the corresponding pixels, all images have similar color) in Row 3rd, Column 2ed, etc. 

\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{1.0\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figure/sscd_mae_selected_bar_v4.pdf}
     \end{subfigure}
     
     \caption{\textbf{Similarity among different unconditional diffusion model settings.} We visualize the quantitative results based upon seven different unconditional diffusion models (DDPMv4, DDPMv6 \citep{ho2020denoising, song2020denoising}, Multistagev1 \citep{multistage}, EDMv1 \citep{karras2022elucidating}, UViT \citep{bao2023all}, CT \citep{song2023consistency}, Progressivev1 \citep{salimans2022progressive}) based upon reproducibility score (left) and MAE score (right) (defined in \Cref{sec:metric}). About more detailed settings and a more comprehensive compare could be found in \Cref{append:unconditional}.}
     \label{fig:reproducibility_selected}
\end{figure}

\subsubsection{Quantitative Studies of Model Reproducibility}
Based upon the setup in \Cref{subsec:uncond-diffusion}, we provide a quantitative study by comparing the similarity metrics of samples generated based upon different network architectures, model perturbation kernels, and training process. In \Cref{fig:reproducibility_selected}, we visualize the \emph{similarity matrix} for seven different popular diffusion models, where each element of the matrix measures pairwise similarities of two different diffusion models based upon reproducibility score (left) and MAE score (right). More comprehensive studies are shown in Appendix \ref{append:unconditional}.
As we can see, there is a very consistent model reproducible phenomenon for comparing any two models. For even the most dissimilar models, (i.e., CT and UViT), the RP and MAE scores are notably high at 0.7 and 0.64, respectively. Specifically, we draw the following conclusions:
\begin{itemize}[leftmargin=*]
    \item \emph{Model reproducibility is consistent among different network architectures.} When comparing DDPMv4, Multistagev1, EDMv1, and UViT, this phenomenon remains consistent regardless of the specific architecture employed.
    \item \emph{Model reproducibility is consistent among different training procedures.} When we compare CT (consistency loss) and EDMv1 (diffusion model loss), even when using different loss functions, they ultimately converge to a similar noise-to-image mapping. Notably, EDMv1 employs a distinct loss by estimating the clear image $\bm x$ whereas other methods estimate the noise $\bm{\epsilon}$. Additionally, comparing DDPMv1 and Progressivev1 reveals that both training from scratch and distillation approaches lead to the same results.
    \item \emph{Model reproducibility is consistent among different sampling procedures.} DDPMv4 utilizes DPM-solver, EDMv1 employs a 2nd order heun-solver, and CT utilizes consistency sampling, yet they all exhibit reproducibility.
    \item \emph{Model reproducibility is consistent among different perturbation kernels.} When compared to DDPMv4, DDPMv6, and EDMv1, the reproducibility remains unaffected by the choice of perturbation method (VP, sub-VP, and VE, respectively).
\end{itemize}

%they still have $70\%$ of generations with SSCD metric larger than 0.6 and $68\%$ of generations with MAE metric smaller than 15.0

  %Notably, in previous work about reproducibility in classification problems \cite{somepalli2022can}, different architectures (e.g. Transformer-based and Convolution Neural Network based) don't converge to the same decision boundary. By comparing CT and EDMv1, with different losses (consistency loss \cite{song2023consistency} and diffusion model loss \cite{karras2022elucidating}), they also converge to a similar noise to image mapping. Also, EDMv1 uses a different loss by estimating the clear image $\rvx_0$ while others estimate the noise $\bm{\epsilon}$. \qq{add to a footnote in architecture}



\begin{figure}[t]
     \centering
     \centering
     \includegraphics[width=1.0\textwidth]{figure/trajectory/manifold_v6.pdf}
     \caption{\textbf{Unqiue Encoding from Noise Hyperplane to Image Manifold.} The diagram illustrates the process of mapping from a noise hyperplane to the image manifold. We employ three distinct models: DDPMv6, EDMv1, and Multistagev1. Initially, we select three different initial noises from Gaussion and generate corresponding samples, denoted by a triangle, square, and circle in the first three images on the left. The hyperplane is defined based on these chosen noises. Image generations, starting from uniformly selected initial noise within this hyperplane, are classified as identical to either the triangle, square, or circle image, determined by the maximum SSCD similarity with them. Each initial noise is colored according to its generation's corresponding class (as indicated on the right; for instance, the noise's generation identical to the triangle image is represented by the black-white color bar), along with the SSCD similarity to the identical image. 
     }
     \label{fig:MappingManifold}
\end{figure}


\subsubsection{Studies of the Unqiue Encoding from Noise Hyperplane to Image Manifold}
The model reproducibility of diffusion models implies that we are learning a unique decoding $f: \mathcal E \mapsto \mathcal I $ from the gaussian noise space $ \mathcal E$ to the image manifold $\mathcal I$. Specifically, we find that  %\qq{emphasize Gaussian for noise space} 
\begin{itemize}[leftmargin=*]
    \item \emph{Similar unique encoding maps across different network architectures.} We further confirm the model reproducibility by visualizing the mapping $f$ from a 2D noise hyperplane $\mathcal H \subseteq \mathcal E$ to the image manifold $\mathcal I$, inspired by \cite{somepalli2022can}. The visualization in \Cref{fig:MappingManifold} shows that different mappings of different network architectures share very similar structures.
    \item \emph{Local Lipschitzness of the unique encoding from noise to image space.} Furthermore, our visualization suggests that the unique encoding $f$ is locally Lipschitz, where $\| f(\bm \eps_1) - f(\bm \eps_2) \| \leq L \| \bm \eps_1 - \bm \eps_2 \|$ for any $\bm \eps_1,\bm \eps_2 \in \mathcal B(\bm \eps, \delta) \cap \mathcal E$ with some Lipschitz constant $L$. Here $\mathcal B(\bm \eps, \delta)$ denotes a ball centered at a Gaussian noise $\bm \eps$ with radius $\delta$. In other words, noises $\bm \eps_1,\bm \eps_2 \in \mathcal E$ close in distance would generate similar reproducible images in $\mathcal I$ via diffusion models.
\end{itemize}

Specifically, the visualization in \Cref{fig:MappingManifold} is created as follows. First, we pick three initial noises $(\bm{\epsilon}_1, \bm{\epsilon}_2, \bm{\epsilon}_3 ) $ in the noise space $\mathcal E$ and used different diffusion model architectures to generate clear images ($\bm x_1$, $\bm x_2$, $\bm x_3$) in the image manifold $\mathcal I$, so that the images $\{\bm x_i\}_{i=1}^3$ belong to three different classes. Second, we create a 2D noise hyperplane with
\begin{align*}
   \bm{\epsilon}\paren{\alpha, \beta} = \alpha \cdot (\bm{\epsilon}_2 - \bm{\epsilon}_1) + \beta \cdot (\bm{\epsilon}_3 - \bm{\epsilon}_1) + \bm{\epsilon}_1
\end{align*}
Within the region $ (\alpha,\beta) \in [-0.1,1.1] \times [-0.1,1,1] $, we uniformly sample $100 $ points along each axis and generate images  $\bm x\paren{\alpha, \beta}$ for each sample $\bm{\epsilon}\paren{\alpha, \beta}$ using different diffusion model architectures (i.e., DDPMv6, EDMv1, Multistagev1). For each point $\paren{\alpha, \beta}$, it is considered as identical to image $\bm x_i$ for $i=\argmax_{k\in\{1, 2, 3\}} [\mathcal{M}_{\text{SSCD}}(\bm x_k, \bm x\paren{\alpha, \beta})]$, and we visualize the value of $\mathcal{M}_{\text{SSCD}}(\bm x_i, \bm x\paren{\alpha, \beta})$. As we observe from \Cref{fig:MappingManifold}, the visualization shares very similar structures across different network architectures. Second, for each plot, closeby noises create images with very high similarities. These observations support our above claims.

%For each point $\bm{\epsilon}\paren{\alpha, \beta}$, we 


%Furthermore, in order to capture the on-manifold behavior from the noise space to generate images' semantics, we create a plane from three random noises and densely create samples on that plane, inspired by the visualization of decision boundary in classification problem \cite{somepalli2022can}. More specifically, we first sample three initial gaussian noise ($\bm{\epsilon}_1, \bm{\epsilon}_2, \bm{\epsilon}_3$) and used different diffusion model architectures to generate clear images ($\rvx_1$, $\rvx_2$, $\rvx_3$). Further, we will generated all images $\rvx_{\alpha \beta}$ from a noise plane $\bm{\epsilon}_{\alpha \beta} = \alpha \cdot (\bm{\epsilon}_2 - \bm{\epsilon}_1) + \beta \cdot (\bm{\epsilon}_3 - \bm{\epsilon}_1) + \bm{\epsilon}_1, -0.1 \leq \alpha, \beta \leq 1.1$ defined by ($\bm{\epsilon}_1, \bm{\epsilon}_2, \bm{\epsilon}_3$). As shown in Fig. \ref{fig:MappingManifold}, we uniformly sampled 100 points along each axis and generated 10k images in total, for each image $\rvx_{\alpha \beta}$, the \textit{Reproducibility Score} is calculated as maximum SSCD metric over three selected clear image $\text{max} [\mathcal{I}_{\text{SSCD}}(\rvx_1, \rvx_{\alpha \beta}), \mathcal{I}_{\text{SSCD}}(\rvx_2, \rvx_{\alpha \beta}), \mathcal{I}_{\text{SSCD}}(\rvx_3, \rvx_{\alpha \beta})]$ and the class it belongs is defined as $\text{argmax} [\mathcal{I}_{\text{SSCD}}(\rvx_1, \rvx_{\alpha \beta}), \mathcal{I}_{\text{SSCD}}(\rvx_2, \rvx_{\alpha \beta}), \mathcal{I}_{\text{SSCD}}(\rvx_3, \rvx_{\alpha \beta})]$. From the figure, we can see that the on-manifold behavior is also very similar for different diffusion model architectures.

%\paragraph{Mapping from Noise Hyperplane to Image Manifold is reproducibility.} \hjz{Originally I just wanted to make this figure as a different way to show the model reproducibility.}

%\paragraph{Local Lipschitz Property of Diffusion Unique Encoding.}



% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figure/gan_vae/gan_nad_vae_v2.pdf}
%          % \caption{Reproducibilty between theoretical and experiment results}
%     \caption{GANS and VAEs \qq{the same as Figure 3, rewrite} }
%     \label{fig:gan_and_vae}
% \end{wrapfigure}

\subsubsection{Comparison with Other Types of Generative Models}
We end this section by highlighting that only diffusion models appear to consistently exhibit model reproducibility. This property is seemingly absent in other generative models with one exception as noted in \cite{khemakhem2020variational}.\footnote{\cite{khemakhem2020variational} demonstrates that VAE is uniquely identifiable encoding given a factorized prior distribution over the latent variables.} In our evaluation of GAN-based methods, we contrast two variants that have been widely used: Wasserstein GAN (wGAN) \cite{arjovsky2017wasserstein} and Spectral Normalization GAN (SNGAN) \cite{miyato2018spectral}. We conduct this analysis using the CIFAR-10 dataset. In the meanwhile, for VAE-based approaches, we consider both the standard VAE and the Variational Autoencoding Mutual Information Bottleneck (VAMP) method \cite{tomczak2018vae}. We evaluate both VAE-based models on the MNIST dataset \cite{lecun1998gradient}. The similarity matrices, presented in \Cref{fig:gan_and_vae}, indicate a lack of model reproducibility in both GAN and VAE based methods.
%Details reproducibility analysis of Generative Adversarial Network (GAN) \cite{goodfellow2014generative} and Variational Autoencoder (VAE) \cite{kingma2013auto} based approaches are in \Cref{append:compare_other_gm}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figure/gan_vae/gan_nad_vae_v4.pdf}
    \caption{\textbf{Quantitative results for GANS and VAEs.} We apply SNGAN, WGAN for the reproducibility evaluation of GAN-based approaches and VAE, VAMP for VAE-based approaches. Each model utilized in this analysis was provided by its respective author, and the reproducibility score is defined the same as in previous experiments. Particularly, the latent space for VAE-based methods is learned through the encoder. In this context, our approach involves sampling initial noise from the latent space of VAE and employing it for the generation of VAMP.}
    \label{fig:gan_and_vae}
\end{figure}

% As a comparison of this observation in the diffusion model, we assess model similarity for both Generative Adversarial Network (GAN) \cite{goodfellow2014generative} and Variational Autoencoder (VAE) \cite{kingma2013auto} based approaches using the reproducibility score. In our evaluation, for GAN-based methods, we contrast wGAN \cite{arjovsky2017wasserstein} and SNGAN \cite{miyato2018spectral} using CIFAR-10. Meanwhile, for VAE-based approaches, we consider both VAE and VAMP \cite{tomczak2018vae} on MNIST dataset \cite{deng2012mnist}. All models are released by the author and the reproducibility score is calculated similarly to the diffusion model. Note that the latent space of the VAE-based method is learned from the encoder, which is different for different models. Here, we sample initial noise from the latent space of one model and use it for the generation of the other. 

% The similarity matrices presented in \Cref{fig:gan_and_vae} imply a lack of reproducibility in both GAN and VAE methods.


% To underscore this observation, we assess model similarity for both Generative Adversarial Network (GAN) \cite{goodfellow2014generative} and Variational Autoencoder (VAE) \cite{kingma2013auto} based approaches using the reproducibility score. In our evaluation, for GAN-based methods, we contrast wGAN \cite{arjovsky2017wasserstein} and SNGAN \cite{miyato2018spectral} using Cifar10. Meanwhile, for VAE-based approaches, we consider both VAE and VAMP \cite{tomczak2018vae} on MNIST. The similarity matrices presented in \Cref{fig:gan_and_vae} imply a lack of reproducibility in both GAN and VAE methods.
% \qq{add a footnote here on conditional VAE, which has reproducibility, if we need space, we can move this paragraph to the appendices}


%In the previous section, the experiments show that uniquely identifiable encoding is a ubiquitous phenomenon among many diffusion model settings. In order to explore whether this phenomenon presents in other powerful, mainstream generative models, we also applied similar experiments on the generative adversarial network (GAN) \cite{goodfellow2014generative} and Variational Autoencoder (VAE) \cite{kingma2013auto}. More specifically, we selected wGAN \cite{arjovsky2017wasserstein}, SNGAN \cite{miyato2018spectral}, VAE, and VAMP \cite{tomczak2018vae} for comparison.

% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[t]{1.0\textwidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/gan_vae/gan_vae_bar.pdf}
%      \end{subfigure}
     
%      \caption{GANS and VAEs}
%      \label{fig:gan_and_vae}
% \end{figure}





% \cite{somepalli2023understanding} using self-supervised copy detection (SSCD) metric \cite{pizzi2022self} to measure the replication between generated images from the diffusion model and the original dataset. Inspired by their setting, we design the \textit{reproducibility score} to measure the replication between two different diffusion models. We randomly sampled 10K noise from the Gaussian distribution and used the same noise for all diffusion models to generate images. For each two diffusion models, we measured the SSCD distance for all image pairs generated from the same noise. Usually, SSCD score above $> 0.4$ reflects a visual replication \cite{somepalli2023understanding}. For \textit{reproducibility score}, it represents the percentage of generation pairs having SSCD similarity $> 0.6$ between two diffusion models. In addition, we also use the mean-absolute-error (MAE) to measure the difference between corresponding image pairs in pixel value space ([0, 255]), and the \textit{MAE score} is reported as the percentage of generation pairs having MAE $< 15.0$ between two diffusion models. The quantitative results for selected diffusion model architectures are shown in Figure \ref{fig:reproducibility_selected}. All quantitative results are shown in Figure \ref{fig:reproducibility_mae_all} and Figure \ref{fig:reproducibility_sscd_all} in Appendix \ref{append:more_results}. Details for different diffusion model settings are shown in Table \ref{tab:unconditional_setting} in Appendix \ref{append:more_results}.




% \begin{figure}
%      \centering
%      \begin{subfigure}[t]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/reproducibility_sscd_selected.png}
%          \caption{reproducibility score}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.45\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/reproducibility_mae_selected.png}
%          \caption{MAE score}
%      \end{subfigure}
%      \caption{Similarity among different unconditional diffusion model settings.}
%      \label{fig:reproducibility_selected}
% \end{figure}












% \begin{figure}
%      \centering
%      \begin{subfigure}[t]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/trajectory/DDPMv6_combine.png}
%          \caption{DDPMv6}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.32\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/trajectory/EDMv1_combine.png}
%          \caption{EDMv1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.32\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/trajectory/Multistagev1_combine.png}
%          \caption{Multistagev1}
%      \end{subfigure}
%      \caption{Mapping Manifold \hjz{need a bar }}
%      \label{fig:MappingManifold}
% \end{figure}








==> section/phenomenon_extension.tex <==
\section{Study Beyond Unconditional Diffusion Models}
\label{sec:reproducibility_more}

%In the preceding sections, we established that model reproducibility is prevalent in the unconditional diffusion model. However, the current landscape of diffusion model applications has evolved towards conditional diffusion models \cite{rombach2022high, ramesh2021zero, nichol2021glide, ho2022classifier, dhariwal2021diffusion}, diffusion model for solving inverse problems \cite{song2023solving,chung2022diffusion,song2021solving, chung2022improving}, diffusion model finetuning \cite{ruiz2023dreambooth, gal2022image, moon2022finetuning, han2023svdiff}, and beyond. 

Furthermore, in this section, we explore how model reproducibility can be generalized to variations of the diffusion models, showcasing that:
\begin{tcolorbox}
\begin{center}
   \textbf{C4:} \emph{Model reproducibility holds \textbf{more generally} across conditional diffusion models, diffusion models for inverse problems, the fine-tuning of diffusion models.} 
\end{center}
\end{tcolorbox}

% \qq{the claim to be two lines}ewq

% \qq{first paragraph: introuduce the general setup, motivation, details postponed to the appendices}

% diffusion models can generalize well to a few images by fine-tuning part of the model 
% and achieving very impressive results. Dreambooth fine-tunes all parameters of the diffusion model except the text transformer and is regularized by generated images. Textual Inversion optimizes only the embedding of a single pseudo-token for each concept while freezing all other parts of the pre-trained model. \cite{moon2022finetuning} fine-tunes the residual and attention blocks of the unconditional diffusion model separately; empirical evidence shows that fine-tuning the attention blocks is less prone to overfitting. \cite{han2023svdiff} reduces the risk of overfitting and language drifting by fine-tuning the singular values of the weight matrices.\cite{xiang2023closer} experiments with different positions for adapter fine-tuning and concludes that the input position after the cross-attention block leads to the best performance. \cite{zhu2022few} fine-tunes the diffusion model with a regularization technique that preserves the relative pairwise distances between synthesized samples. In this section, we are going to explore whether the diffusion model still has the same uniquely identifiable encoding when being a conditional diffusion model \ref{sec:reproducibility_conditional}, projection-based diffusion model \ref{sec:reproducibility_projectionbased}, and fine-tuning for diffusion model \ref{sec:reproducibility_fintuning}.



\subsection{Model Reproducibility in Conditional Diffusion Models} 
Conditional diffusion, introduced by \cite{ho2022classifier, dhariwal2021diffusion}, gained its popularity in many applications such as text-to-image generation  \citep{rombach2022high, ramesh2021zero, nichol2021glide} with superior performance, through the fusion of rich class embeddings with the denoiser function. Interestingly, we find that:
\begin{center}

    \emph{Model reproducibility of conditional models is evident and linked with unconditional counterparts.}

\end{center}
Specifically, our experiments in \Cref{fig:rp_conditional} demonstrate that (\emph{i}) model reproducibility exists among different conditional diffusion models, and (\emph{ii}) model reproducibility is present between conditional and unconditional diffusion models \emph{only} if the type (or class) of content generated by the unconditional models matches that of the conditional models. More results can be found in  \Cref{append:conditional}. 

To support our claims, we introduce the \emph{conditional reproducibility score} between different conditional diffusion models by $\text{RP}_{cond} \text{ Score} := \mathbb{P}\paren{\mathcal{M}_{\text{SSCD}}(\bm x^c_1, \bm x^c_2)>0.6 \mid c \in \mathcal C }$, where the pair $(\bm x^c_1, \bm x^c_2)$ are generated by two conditional models from the same initial noise and conditioned on the class $c\in \mathcal C$. Additionally, the \emph{between reproducibility score} of conditional and unconditional diffusion models is defined as $\text{RP}_{between} \text{ Score}:= \mathbb{P}\paren{\max_{_{c \in \mathcal C}}[\mathcal{M}_{\text{SSCD}}(\bm x_1, \bm x^c_2)]>0.6}$, for an unconditional generation $\bm x_1$ and conditional generation $\bm x^c_2$ starting from the same noise. First, when conditioned on the same class and initial noise, results in \Cref{fig:rp_conditional} (a) (b)
highlight the similarity of samples generated from different condition diffusion models (i.e., EDM-cond, UViT-cond, and MultistageEDM-cond), supporting Claim (\emph{i}). Second, the high $\text{RP}_{between} \text{ Score}$ in \Cref{fig:rp_conditional} (c) provides strong evidence for reproducibility between conditional and unconditional diffusion models, supporting Claim (\emph{ii}). This can also be observed visually by examining the unconditional generation using Progressivev1 in \Cref{fig:rp_conditional} (a), where images highlighted in the green square share high similarity with conditional counterparts highlighted in the purple square .

%unconditional generation results using Progressivev1 and 

%Furthermore, when examining unconditional generation results (Progressivev1) in \Cref{fig:rp_conditional} (a), a striking resemblance is observed between these results and conditional generation samples within the same class and initial noise (highlighted in the red square). Additional results can be found in \Cref{append:unconditional} and \Cref{append:conditional}. 



%We investigate the model reproducibility for (1) within conditional diffusion models; (2) between conditional and unconditional diffusion models.
%The reproducibility score between conditional diffusion models is defined as $\text{RP Score} := \mathbb{P}\paren{\mathcal{M}_{\text{SSCD}}(\bm x^c_1, \bm x^c_2)>0.6 \mid c \in \mathcal C }$, for generation pairs $(\bm x^c_1, \bm x^c_2)$ generated by two conditional model from the same initial noise and conditioned on $c$, which belongs to the classes set $\mathcal C$ from the dataset. The reproducibility score between the conditional diffusion model and the unconditional diffusion model is defined as $\text{RP Score}:= \mathbb{P}\paren{\max_{_{c \in \mathcal C}}[\mathcal{M}_{\text{SSCD}}(\bm x_1, \bm x^c_2)]>0.6}$, for an unconditional generation $\bm x_1$ and conditional generation $\bm x^c_2$ from the same initial noise. Results are shown in \Cref{fig:rp_conditional}.

% \begin{itemize}[leftmargin=*]
%     \item \emph{Model reproducibility exists across conditional diffusion models and could be extended between conditional diffusion models and unconditional models in a special way.} From the information presented in  \Cref{fig:rp_conditional} (a), it is evident that when considering generation samples produced by EDM-cond, UViT-cond, and MultistageEDM-cond given the same class and initial noise, there is a notable similarity observed. More results can be found in the attached section labeled \Cref{append:conditional}. Furthermore, it is worth noting that the reproducibility score among these various diffusion models is consistently high, with a minimum value of 0.77 (between UViT-cond and MultistageEDM-cond) in \Cref{fig:rp_conditional} (b). This high reproducibility score serves as evidence for the existence of reproducibility within conditional diffusion models. What adds to the intrigue is that when examining the generation results from the unconditional diffusion model (Progressivev1) shown in \Cref{fig:rp_conditional} (a), considering all generated samples within class 0 (e.g., the class "plane," which is the same class used for conditional generation), they bear a striking resemblance to the conditional generation samples with the same class and initial noise. (those samples are highlighted in the red square). More results could be found in \Cref{append:unconditional} and \Cref{append:conditional}. To provide a quantitative demonstration of this relationship, we made modifications to the reproducibility score (details are in \Cref{append:conditional}). The resulting scores are displayed in \Cref{fig:rp_conditional} (c). And the consistently high reproducibility score observed between conditional and unconditional diffusion models serves as strong evidence of reproducibility existing between these two model types. 
% \end{itemize}

\begin{figure}[t]
     \centering
     \includegraphics[width=1.0\linewidth]{figure/conditional_sample/con_uncon_final.pdf}
     \caption{\textbf{Model reproducibility for conditional diffusion model.} In this study, we employ conditional diffusion models, specifically U-Net-based (EDM-cond, MultistageEDM-cond) and transformer based (UViT-cond), which we train on the CIFAR-10 dataset using class labels as conditions.  Additionally, we select unconditional diffusion models, namely Progressivev1, DDPMv4, and EDMv2, as introduced in  \Cref{sec:uncond}. Figure (a) showcases sample generations from both unconditional and conditional diffusion models (with the "plane" serving as the condition for the latter). Notably, samples within the same row and column originate from the same initial noise. The reproducibility scores between the conditional diffusion models are presented in (b), and between unconditional and conditional diffusion models in (c).}
     \label{fig:rp_conditional}
\end{figure}



\subsection{Model Reproducibility in Solving Inverse Problems}
Recently, diffusion models have also demonstrated remarkable results on solving a broad spectrum of inverse problems \citep{song2023solving, chung2022diffusion, song2021solving, chung2022improving},\footnote{Here, the problem is often to reconstruct an unknown signal $\bm u$ from the measurements $\bm z$ of the form $\bm z = \mathcal{A}(\bm u) + \bm \eta$, where $\mathcal{A}$ denotes some (given) sensing operator and $\bm \eta$ is the noise.} including but not limited to image super-resolution, de-blurring, and inpainting. Motivated by these promising results, we illustrate based upon solving the image inpainting problem using a modified deterministic variant of diffusion posterior sampling (DPS) \citep{chung2022diffusion}, showcasing that for solving inverse problem using diffusion models:
\begin{center}

    \emph{Model reproducibility largely holds only within the same type of network architectures.} 

\end{center}
Our claim is supported by the experimental results in \Cref{fig:rp_inverseproblem}.
Specifically, \Cref{fig:rp_inverseproblem} (a) virtualizes the samples generated from different diffusion models, and \Cref{fig:rp_inverseproblem} (b) presents the similarity matrix of model reproducibility between different models, i.e., U-Net based (DDPMv1, DDPMv2, DDPMv3, DDPMv4, Multistagev1) and Transformer based (DiT, U-ViT) architectures. We note a strong degree of model reproducibility \emph{among} architectures of the same type (such as U-Net or Transformer), but the model reproducibility score exhibits a notable decrease when comparing any U-Net model to any Transformer-based model.

%\Cref{fig:rp_inverseproblem} (a), (b) demonstrates notably higher reproducibility scores within the same type of architectures, compared to scores between these types. This underscores the persistence of model reproducibility within the same type of architecture and its decline between different types of architectures in solving inverse problems.

%The utilization of methods such as those presented in \cite{song2023solving, chung2022diffusion, song2021solving, chung2022improving} empowers unconditional diffusion models to effectively address a broad spectrum of diverse inverse problems (e.g. image super-resolution, de-blurring, inpainting, and so on), all without the necessity of additional training. In the context of our analysis, we focus on comparing the generation of samples originating from identical initial noise and observations $\bm z$ (as depicted in \Cref{fig:rp_inverseproblem}) for the specific task of image inpainting. We observe that,

% \begin{itemize}[leftmargin=*]
%     \item \emph{Model reproducibility exists within similar architectures but diminishes across different architectures for inverse problem-solving.} From the outcomes depicted in  \Cref{fig:rp_inverseproblem} (a), when considering the observations $\bm y$, it is apparent that while the generated results do not consistently resemble the unknown signal $\bm x$ for various initial noise, there remains reproducibility when starting from the same initial noise within different diffusion models. However, a more detailed examination of the generation reveals that the generated results exhibit a greater degree of similarity within architecture categories, such as U-Net-based (DDPMv1, DDPMv2) and Transformer-based (DiT, U-ViT) architectures, e.g. the sample in the first row and first column for each diffusion model. Furthermore, as shown in \Cref{fig:rp_inverseproblem} (b), it is evident that the reproducibility scores are significantly higher within U-Net-based architectures (DDPMv1, DDPMv2, DDPMv3, DDPMv4, Multistagev1) and Transformer-based architectures (DiT, U-ViT) compared to the reproducibility scores between these two architectural categories. This underscores that model reproducibility persists within similar architectures but diminishes when transitioning across different architectural paradigms when solving inverse problems.
% \end{itemize}


% From the outcomes depicted in  \Cref{fig:rp_inverseproblem} (a), when considering the observations $\bm z$, it is apparent that while the generated results do not consistently resemble the unknown signal $\bm u$ for various initial noise, there remains reproducibility when starting from the same initial noise within different diffusion models. However, a more detailed examination of the generation reveals that the generated results exhibit a greater degree of similarity within architecture categories, such as U-Net-based (DDPMv1, DDPMv2) and Transformer-based (DiT, U-ViT) architectures, e.g. the sample in the first row and first column for each diffusion model. Furthermore, as shown in \Cref{fig:rp_inverseproblem} (b), it is evident that the reproducibility scores are significantly higher within U-Net-based architectures (DDPMv1, DDPMv2, DDPMv3, DDPMv4, Multistagev1) and Transformer-based architectures (DiT, U-ViT) compared to the reproducibility scores between these two architectural categories. This underscores that model reproducibility persists within similar architectures but diminishes when transitioning across different architectural paradigms when solving inverse problems.

\begin{figure}[t]
     \centering
     \includegraphics[width=1.0\linewidth]{figure/inpainting_sample/inpainting_img_2_v2.pdf}
     \caption{\textbf{Model reproducibility for solving inverse problems.} In this investigation, we employ various unconditional diffusion models, as introduced in \Cref{sec:uncond}, which were initially trained on the CIFAR-10 dataset. Our approach involves utilizing a modified deterministic variant of diffusion posterior sampling (DPS), as detailed in \Cref{append:inverseproblem}. Specifically, we focus on the task of image inpainting. Figure (a) presents both the observation $\bm z$, unknown signal $\bm u$, and generations from different diffusion models. Notably, samples within the same row and column originate from the same initial noise. The reproducibility scores for the generated outputs from different diffusion models under the DPS algorithm are quantitatively analyzed in (b).}
     \label{fig:rp_inverseproblem}
\end{figure}



\subsection{Model Reproducibility in Fine-tuning Diffusion Models} Few-shot image fine-tuning for diffusion models, as discussed in \citep{ruiz2023dreambooth, gal2022image, moon2022finetuning, han2023svdiff}, showcases remarkable generalizability. This is often achieved by fine-tuning a small portion of the parameters of a large-scale pre-trained (text-to-image) diffusion model. In this final study, we delve into the impacts of partial model fine-tuning on both model reproducibility and generalizability, by extending our analysis in \Cref{sec:analysis}. We show that:
\begin{center}

    \textit{Partial fine-tuning reduces reproducibility but improves generalizability in ``memorization regime''.}

\end{center}
Our claim is supported our results in \Cref{fig:rp_finetuning}, comparing model fine-tuning and training from scratch of with varying size of the training data, where both models have the same number of parameters. In comparison to training from scratch that we studied in \Cref{fig:regime}, fine-tuning specific components of pre-trained diffusion models, particularly the attention layer in the U-Net architecture, yields lower model reproducibility score but higher generalization score in the memorization regime. However, in the generalization regime, partial model fine-tuning has a minor impact on both reproducibility and generalization in the diffusion model.
Our result reconfirms the improved generalizability of fine-tuning diffusion models on limited data, but shows a surprising tradeoff in terms of model reproducibility that is worth of further investigations.
%within diffusion models trained on datasets of varying sizes, as depicted in Figure,

 %Contrary to the scenario in \Cref{fig:regime}, where training diffusion models from scratch in the memorization regime results in high reproducibility but low generalization scores, fine-tuning specific components, particularly the attention layer in the U-Net architecture, yields low reproducibility but high generalization scores. This demonstrates that within the memorization regime, characterized by limited dataset sizes, partial model fine-tuning reduces reproducibility while improving generalization.

\begin{figure}[t]
     \centering

     \begin{subfigure}[t]{1.0\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figure/fintuning_sample/reproducibility_finetuning_v2.pdf}
         % \caption{Reproducibilty}
         \label{fig:reproducibility_finetuning}
     \end{subfigure}
     % \hfill

     \caption{\textbf{Model reproducibility for diffusion model finetuing.} In this experiment, we employ DDPMv4. Two distinct training strategies are investigated: "from scratch," denoting direct training on a subset of the CIFAR-10 dataset, and "partial fine-tuning," which involves pretraining on the entire CIFAR-100 dataset \cite{krizhevsky2009learning} followed by fine-tuning only the attention layers of the model on a subset of the CIFAR-10 dataset. The dataset sizes for CIFAR-10 range from $2^6$ to $2^{15}$. Importantly, both "from scratch" and "partial fine-tuning" are trained using the same subset of images for each dataset size. Under different dataset sieze, Figure (a) illustrates the reproducibility score between these two strategies and (b) presents the generalization score for them.}    
     \label{fig:rp_finetuning}
\end{figure}

% \begin{figure}[htbp]
%      \centering
%      \begin{subfigure}[t]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/fintuning_sample/comparion_finetuning.png}
%          \caption{Reproducibilty}
%          \label{fig:reproducibility_finetuning}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/fintuning_sample/comparion_finetuning_generalization.png}
%          \caption{Generalizability}
%          \label{fig:generalizability_finetuning}
%      \end{subfigure}
%      \hfill
%      \caption{\textbf{Reproducibility for diffusion model finetuing.} We utilize U-Net based diffusion models \cite{song2020score} for this experiment. "from scratch" represents direct training on a subset of the CIFAR-10 dataset \cite{krizhevsky2009learning}, "partial finetuning" represents first pretraining on the entire CIFAR-100 dataset and then finetuning only the attention layers of the model on a subset of CIFAR-10 dataset. The dataset size of CIFAR-10 ranging from $2^6$ to $2^{15}$. Under each dataset size, both "from scratch" and "partial finetuning" are trained from the same subset of images. (a) displays the reproducibility score between these two diffusion model training settings under the same dataset size. (b) displays the generalization score for each diffusion model training setting under different dataset sizes.}    
%      \label{fig:rp_finetuning}
% \end{figure}



% \qq{put all the experiment setups into the caption of each figure}


% Although reproducibility is ubiquitous in the unconditional diffusion model, nowadays more fancy diffusion model applications do not employ the unconditional diffusion model. \hjz{Need more related work} Nowadays, most of the state-of-art diffusion models are conditional diffusion models, especially some large diffusion model like Stable Diffusion \cite{rombach2022high}, DALL$\cdot$E \cite{ramesh2021zero}, GLIDE \cite{nichol2021glide}. \cite{song2023solving,chung2022diffusion,song2021solving} utilize diffusion model to solve inverse problems by \hjz{might not accurate} global hard consistency or projection-based local consistency, display the superiority of using diffusion model to solve inverse problems. Dreambooth \cite{ruiz2023dreambooth} and Textual Inversion \cite{gal2022image} 
% diffusion models can generalize well to a few images by fine-tuning part of the model 
% and achieving very impressive results. Dreambooth fine-tunes all parameters of the diffusion model except the text transformer and is regularized by generated images. Textual Inversion optimizes only the embedding of a single pseudo-token for each concept while freezing all other parts of the pre-trained model. \cite{moon2022finetuning} fine-tunes the residual and attention blocks of the unconditional diffusion model separately; empirical evidence shows that fine-tuning the attention blocks is less prone to overfitting. \cite{han2023svdiff} reduces the risk of overfitting and language drifting by fine-tuning the singular values of the weight matrices.\cite{xiang2023closer} experiments with different positions for adapter fine-tuning and concludes that the input position after the cross-attention block leads to the best performance. \cite{zhu2022few} fine-tunes the diffusion model with a regularization technique that preserves the relative pairwise distances between synthesized samples. In this section, we are going to explore whether the diffusion model still has the same uniquely identifiable encoding when being a conditional diffusion model \ref{sec:reproducibility_conditional}, projection-based diffusion model \ref{sec:reproducibility_projectionbased}, and fine-tuning for diffusion model \ref{sec:reproducibility_fintuning}.

% \subsection{Conditional Diffusion Model}

% \textbf{Experiment setting} To investigate the reproducibility of the conditional diffusion model, we choose three architectures, conditional EDM \cite{karras2022elucidating}, conditional multistage EDM \hjz{cite multistage}, and conditional U-ViT \cite{bao2023all}. We used the CIFAR-10 dataset for training and used their labels as conditions.  The difference between EDM and multistage EDM is only the architecture of the score function. But the difference between EDM and conditional U-ViT is not only the architecture but also the way they embed the conditional. EDM uses a one-hot label for embedding and the feature is embedding by Multilayer Perceptron (MLP) but the condition for U-Vit is embedded through a lookup table with fixed embeddings. For all three architectures, we train them till convergence (achieved the lowest FID). To generate the sample, we use the same 10K initial noise as the one for the unconditional setting (Section \ref{sec:reproducibility_unconditional}), and for each initial noise, we generate 10 images guided by 10 classes, which is 100K image in total. The \textit{reproducibility score} is reported as the mean of all classes. Also, we defined \textit{reproducibility score} between the conditional diffusion model and the unconditional diffusion model. For each initial noise, we will use the conditional diffusion model to generate samples in all classes and use the unconditional diffusion model to generate one sample, the SSCD similarity for this initial noise is the minimum SSCD similarity between the image from unconditional diffusion model and all images from conditional diffusion model. The overall \textit{reproducibility score} for those two models is the perception of generation pairs having SSCD similarity $>$ 0.6.

% As shown in Figure \ref{fig:unconditional_sample} (a, b, c) and Figure \ref{fig:reproducibility_conditional} (a), the reproducibility phenomenon still appears in the conditional diffusion model setting. What's more interesting is the relationship between the unconditional and conditional diffusion models. For the unconditional diffusion model (CT in \ref{fig:unconditional_sample}(d)), all generated samples in class 0 (class plane) are highlighted in red square. And for those images, they are very similar to the conditional generation with the same initial noise (same row and column in the figure) and class 0. What's more, if you compare the generation of the unconditional diffusion model in other classes to the conditional setting in Appendix the \textit{reproducibility score} between the selected conditional diffusion model and the unconditional diffusion model in Appendix \ref{appendix:conditional}, you will have similar findings. The quantitative analysis is shown in Figure \label{fig:reproducibility_conditional} (b), the high \textit{reproducibility score} between unconditional and conditional diffusion models indicates that for each initial noise, let conditional diffusion model generate the sample for each class, and the corresponding unconditional generation should be one of them.


% \begin{figure}[htbp]
%      \centering
%      \begin{subfigure}[t]{0.24\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/conditional_sample/edm_cond_0.png}
%          \caption{EDM}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.24\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/conditional_sample/edm_mul_cond_0.png}
%          \caption{MultistageEDM}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.24\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/conditional_sample/uvit_cond_0.png}
%          \caption{U-ViT}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.24\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/conditional_sample/ct_compare.png}
%          \caption{Unconditional CT}
%      \end{subfigure}
%      \caption{Conditional diffusion model samples visualization (class 0) and comparison of unconditional diffusion model. Samples in the corresponding row and column are generated from the same initial noise, for both conditional and unconditional models.}
%      \label{fig:unconditional_sample-conditional}
% \end{figure}

% \begin{figure}
%      \centering
%      \begin{subfigure}[t]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/conditional_sample/reproducibility_cond.png}
%          \caption{Conditional diffusion models}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.45\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/conditional_sample/reproducibility_cond_uncond.png}
%          \caption{Conditional and unconditional diffusion model}
%      \end{subfigure}
%      \caption{reproducibility among different conditional diffusion model settings and their relationship with unconditional diffusion model}
%      \label{fig:reproducibility_conditional}
% \end{figure}

% \begin{figure}
%      \centering
%      \includegraphics[width=0.75\linewidth]{figure/conditional_sample/uncon_con_with_bar.pdf}
%      \caption{\textbf{Reproducibility for conditional diffusion model.}}
%      \label{fig:reproducibility_conditional}
% \end{figure}

% \label{sec:reproducibility_conditional}

% \subsection{Diffusion Model for inverse problem solving} 

% \label{sec:reproducibility_inverseproblem}

% \begin{figure}
%      \centering
%      \includegraphics[width=\linewidth]{figure/inpainting_sample/inpating_with_bar.pdf}
%      \caption{Easy inpainting}
%      \label{fig:reproducibility_inverseproblem}
% \end{figure}

% \subsection{Fintuning for Diffusion Model}

% \label{sec:reproducibility_fintuning}



% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[t]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/fintuning_sample/comparion_finetuning.png}
%          \caption{Reproducibilty}
%          \label{fig:reproducibility_finetuning}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figure/fintuning_sample/comparion_finetuning_generalization.png}
%          \caption{Generalizability}
%          \label{fig:generalizability_finetuning}
%      \end{subfigure}
%      \hfill
%      \caption{Finetuing}    
%      \label{fig:theoretical_analysis}
% \end{figure}

==> section/reproducibility_statement.tex <==
\begin{center}
{\Large \bf Reproducibility Statement}
\end{center}

\startcontents[sections]
\printcontents[sections]{l}{1}{\setcounter{tocdepth}{2}}


To illustrate the intriguing phenomenon of consistent model reproducibility, there is no requirement to provide any code or model for validation. The only thing provided is the initial random noise we used for the 8$\times$8 image grid. By selecting one diffusion mode list in the paper (you could also explore other diffusion models not listed in the paper), you can access their released model online. The only prerequisite is that the training dataset should be CIFAR-10.  By following this approach, you could regenerate the samples for unconditional in \Cref{fig:unconditional_sample},\ref{appendfig:uncond_vis_all} and for conditional in \Cref{appendfig:conditional_vis_1}, \ref{appendfig:conditional_vis_2}. The details of the experiment for the unconditional model are in \ref{append:unconditional}, for the conditional diffusion model are in \ref{append:conditional}, for theoretical verification are in \ref{append:theory}, for diffusion models on inverse problems solving are in \ref{append:inverseproblem} and for fine-tuning diffusion models are in \ref{append:fintuning}.

==> section/theory.tex <==
\section{Correlation between Reproducibility \& Generalizability}
\label{sec:analysis}
%\subsection{Diffusion model could be proved as uniquely identifiable encoding}

   %  We design experiments to see the effect of training dataset size and model capacity on the convergence to the theoretical solution. We use the CIFAR-10 dataset by selecting part of their images to change the training dataset size. We use UNet from \cite{song2020score} as the architecture for the score function, and we change the model capacity by changing the embedding dimension. As shown in Figure \ref{fig:theoretical_analysis}, e.g. UNet-128 represents a UNet architecture with 128 embedding dimensions. To evaluate the convergence to the optimal solution, we use both theoretical score functions in Theorem \ref{theorem:optimal_regression} and our training diffusion model to generate 10K samples and calculate the reproducibility score, as shown on the left of Figure \ref{fig:theoretical_analysis}. We also compare the reproducibility score between models with different parameter numbers, shown in the middle of Figure \ref{fig:theoretical_analysis}. On the right of Figure \ref{fig:theoretical_analysis}, we also show the generalizability of different training settings. Similar to \cite{somepalli2023understanding}, for each generated image, we compare its SSCD similarity with the entire training dataset. }
  
 

More interestingly, both of our empirical and theoretical studies in this section demonstrate that 
\begin{tcolorbox}
\begin{center}
   \textbf{C3:} \emph{The consistent model reproducibility of diffusion models manifests in two distinct training regimes, both \textbf{strongly correlated} with the model's generalizability.}
\end{center}
\end{tcolorbox}
Here, the model's generalizability means the model's ability to generate new samples that is different from samples in the training dataset.
Specifically, we measure the generalizability by introducing the \textit{generalization (GL) score} $:=1 - \mathbb{P}\paren{\max_{i\in[N]} \left[\mathcal{M}_{\text{SSCD}}(\bm x, \bm y_i)\right]>0.6}$ represents one minus the \emph{probability} of maximum $\mathcal{M}_{\text{SSCD}}$ is larger than $0.6$,  between the generated sample $\bm x$ from one diffusion model and all samples $\bm y_i$ from training dataset $\Brac{\bm y_i }_{i=1}^N $ of $N$-samples. We sampled 10K initial noise to estimate the probability. 

% \begin{align*}
%     \text{GL score} \;:=\; 1 - \mathbb{P}\paren{\max\limits_{i\in[N]} \left[\mathcal{M}_{\text{SSCD}}(\bm x, \bm y_i)\right]>0.6},
% \end{align*}
\subsection{Two Regimes of Model Reproducibility} 
Now, we formally introduce the two regimes of model reproducibility for diffusion models in the following. Both of them exhibit a strong correlation with the model's ability to generalize.
%\qq{maybe we need to compare the model size vs the training data size to claim overparameterization and underparameterization? The straight lines can be drawn based upon overparmeterization and under parameterization}
%\qq{rephrase the following, overparameterization}
\begin{itemize}[leftmargin=*]
    \item \textbf{``Memorization regime''} characterizes a scenario where the trained model has large model capacity than the size of training data. In this regime, starting from the same noise the model possesses the ability to reproduce the same results, as illustrated in the left region of \Cref{fig:reproducibility} with small training data size. However, the generated samples are often replications of the samples in the training data, and the model lacks the full capacity to generate new samples; see the left region of \Cref{fig:regime}. Therefore, we call this regime the ``memorization regime'' as the generated samples are only replication of training data. In this regime, we can rigorously characterize the optimal denoiser as shown in \Cref{theorem:unique_identitical_encoding}, and in \Cref{fig:theoretical_verification} we empirically demonstrated that the diffusion models converge to the theoretical solutions when the model is highly overparameterized. However, given no generalizability, training diffusion models in this regime holds limited practical interest.

    \item \textbf{``Generalization regime''} emerges when the diffusion model is trained on large dataset and doesn't have full capacity to memorize the whole dataset. Remarkably, as shown in the right region of \Cref{fig:reproducibility}, the diffusion model regains the reproducibility as the ratio between dataset size and model capacity increases. Simultaneously, the model possess the ability to generate new samples, as illustrated in the right region of \Cref{fig:regime}; this generalization phenomenon is also observed in \cite{yoon2023diffusion}. As such, we call this regime the ``generalization regime'' because the stage of generalization is in coincidence with the stage of model reproducibility. This is the regime in which diffusion models are commonly trained and employed in practice, and the coexistence of model reproducibility and generalizability is an intriguing phenomenon to be further understood theoretically. 
\end{itemize}


%\textbf{(a) ``memorization regime''} characterizes a scenario where the model is overparameterized and trained on a small dataset. In this regime, while the model possesses the ability to reproduce the same results (\Cref{fig:reproducibility}, left region) starting from the same noise, the generated data is often a replication of samples in the training data, and the model lacks the full capacity to generate new samples (\Cref{fig:regime}, left region). Although this regime holds limited practical interest,  we rigorously characterized the global solution, and demonstrated that the diffusion models will reproduce the theoretical solutions. Conversely,  

%\qq{combine the two theories below}
% \qq{change theta to be bold, all symbols to be italic}
\subsection{A Theoretical Study of the Memorization Regime} 
For the rest of this section, we provide a theoretical study of the memorization regime, and we leave the study of generalization regime for future work. Specifically, we characterize the optimal denoiser of the diffusion model and show that it results in a unique identifiable encoding under proper assumptions.


% \begin{wrapfigure}{r}{0.5\textwidth}
%     \begin{center}
%     \includegraphics[width=.8\linewidth]{figure/analysis/comparion_theoratical_v5.png}
%     \end{center}
%     \caption{\textbf{Experiment verification of the theory.} We employ DDPMv4 and conduct training on the CIFAR-10 dataset. During this process, we make modifications to both the model's capacity and the size of the training dataset, maintaining the same configuration as depicted in \Cref{fig:theoretical_analysis}. The figure presented here illustrates the reproducibility score between each diffusion model and the theoretically unique identifiable encoding as outlined in \Cref{theorem:unique_identitical_encoding}.}
%     \label{fig:theoretical_verification}
% \end{wrapfigure}
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.5\linewidth]{figure/analysis/comparion_theoratical_v5.png}
    \end{center}
    \caption{\textbf{Experiment verification of the theory.} We employ DDPMv4 and conduct training on the CIFAR-10 dataset. During this process, we make modifications to both the model's capacity and the size of the training dataset, maintaining the same configuration as depicted in \Cref{fig:theoretical_analysis}. The figure presented here illustrates the reproducibility score between each diffusion model and the theoretically unique identifiable encoding as outlined in \Cref{theorem:unique_identitical_encoding}.}
    \label{fig:theoretical_verification}
\end{figure}

\begin{theorem}\label{theorem:unique_identitical_encoding}
    Suppose we train a diffusion model denoiser function $\bm \eps_{\bm \theta} (\bm x,t)$ with parameter $\bm \theta$ on a training dataset $\Brac{\bm y_i }_{i=1}^N $ of $N$-samples, by minimizing the training loss
    \begin{align}\label{eqn:training-loss}
       \min_{\bm \theta}  \mathcal{L}(\bm{\epsilon}_{\bm{\theta}}; t) = \mathbb{E}_{\bm x_0 \sim p_{\text{data}}(\bm x)}\mathbb{E}_{\bm x \sim p_{t}(\bm x|\bm x_0)} [||\bm{\epsilon} - \bm{\epsilon}_{\bm{\theta}}(\bm x, t)||^2],
    \end{align}
    where we assume that data $\bm x_0$ follows a mixture delta distribution $p_{\text{data}}(\bm x) = \frac{1}{N} \sum_{i =1}^{N} \delta (\bm x - \bm y_i)$, and the perturbation kernel $p_{t}(\bm x_t|\bm x_0) = \mathcal{N}(\bm x_t;s_t\bm x_0, s_t^2\sigma_t^2\textbf{I})$ with perturbation parameters $s_t, \sigma_t$. Then we can show that the optimal denoiser $ \bm{\epsilon}^*_{\bm{\theta}}(\bm x;t) = \argmin_{\bm{\epsilon}_{\bm{\theta}}} \mathcal{L}(\bm{\epsilon}_{\bm{\theta}}; t)$ is 
\begin{align}\label{eqn:optimal-eps}
    \bm{\epsilon}^*_{\bm \theta}(\bm x;t) = \frac{1}{s_t\sigma_t}\brac{\bm x - s_t\frac{\sum_{i = 1}^{N}\mathcal{N}(\bm x;s_t\bm y_i, s_t^2\sigma_t^2\textbf{I})\bm y_i}{\sum_{i = 1}^{N}\mathcal{N}(\bm x;s_t\bm y_i, s_t^2\sigma_t^2\textbf{I})}}.
\end{align}
Moreover, suppose a trained diffusion model could converge to the optimal denoiser $\bm{\epsilon}^*_{\bm \theta}(\bm x;t)$ and we use a deterministic ODE sampler to generate images using $ \bm{\epsilon}^*_{\bm \theta}(\bm x;t) $, then $f: \mathcal E \mapsto \mathcal I$, which is determined by the $\bm{\epsilon}^*_{\bm \theta}(\bm x;t)$ and the ODE sampler, is an invertiable mapping and the inverse mapping $f^{-1}$ is a unique identifiable encoding. %\hjz{How detailed}. \qq{do we have an analyatic form of $f$? otherwise, this might be good enough}
  %  with a mixture delta distribution $p_{\text{data}}(\rvx) = \frac{1}{N} \sum_{i =1}^{N} \delta (\rvx - \rvy_i)$ and perturbation kernel $p_{t}(\rvx_t|\rvx_0) = \mathcal{N}(\rvx_t;s_t\rvx_0, s_t^2\sigma_t^2\textbf{I})$
\end{theorem}


%\begin{theorem}
%\label{theorem:optimal_regression}
%Given a diffusion model process trained on a dataset with $Y$ samples $\rvy_{i\in[Y]}$, modeled as a mixture delta distribution $p_{\text{data}}(\rvx) = \frac{1}{Y} \sum_{i =1}^{Y} \delta (\rvx - \rvy_i)$,  perturbation kernel $p_{t}(\rvx_t|\rvx_0) = \mathcal{N}(\rvx_t;s_t\rvx_0, s_t^2\sigma_t^2\textbf{I})$, training loss $\mathcal{L}(\bm{\epsilon}_\theta; t) = \mathbb{E}_{\rvx_0 \sim p_{\text{data}}(\rvx)}\mathbb{E}_{\rvx \sim p_{t}(\rvx|\rvx_0)} [||\bm{\epsilon} - \bm{\epsilon}_\theta(\rvx, t)||^2]$, the optimal regression function could be proved as $\bm{\epsilon}^*_\theta(\rvx;t) = \frac{1}{s_t\sigma_t}[\rvx - s_t\frac{\sum_{i = 1}^{Y}\mathcal{N}(\rvx;s_t\rvy_i, s_t^2\sigma_t^2\textbf{I})\rvy_i}{\sum_{i = 1}^{Y}\mathcal{N}(\rvx;s_t\rvy_i, s_t^2\sigma_t^2\textbf{I})}]$.

%Suppose a diffusion model could converge to the optimal regression function, and given a deterministic ODE sampler, it should be uniquely identifiable encoding. \qq{xx}
%\end{theorem}

%\begin{theorem}
%\label{theorem:unique_identitical_encoding}
%Suppose a diffusion model could converge to the optimal regression function, and given a deterministic ODE sampler, it should be uniquely identifiable encoding.
%\end{theorem}



The proof for \Cref{theorem:unique_identitical_encoding} can be found in the \Cref{append:theory}, building upon previous findings from \cite{karras2022elucidating, yi2023generalization}. It is worth noting that the optimal denoiser $ \bm{\epsilon}^*_{\bm \theta}(\bm x;t)$ in (\ref{eqn:optimal-eps}) is deterministic for a given training dataset $\Brac{\bm y_i }_{i=1}^N $ and for specific perturbation parameters $s_t, \sigma_t$. Moreover, \cite{yi2023generalization} demonstrates optimal denoiser lacks generalizability, as all the samples generated from $\bm{\epsilon}^*_{\bm \theta}(\bm x;t)$ are confined within the training dataset. Furthermore, we verified our theory experimentally by comparing the reproducibility score between the 
the theoretical generations in \Cref{theorem:unique_identitical_encoding} and that of a trained network in practice. This can be illustrated by the left region of \Cref{fig:theoretical_verification}, the trained networks have a very high similarity compared with the theoretical solution on small training dataset, and the similarity decreases when the size of training data increases. As such, we conclude that the diffusion model could converge to the theoretical solution when the model capacity is large enough. 

 
%\qq{rephrase the sentences in the following} From \Cref{fig:theoretical_analysis-main}, we could find when the dataset size is small, our experiments have a very high similarity compared with the theoretical solution. As the dataset size increases or the model capacity decreases, the model becomes harder to converge to the theoretical solution. we conclude that the diffusion model could converge to the theoretical solution when the model capacity is enough.

%\qq{add more dicussion and conclusion here; generalization regime discussion; for future work}


%However, previous work \cite{yi2023generalization} shows that this optimal regression function has no generalizability (all the samples generated from the optimal function are from the dataset),
%and the diffusion model could not converge to this optimal regression function.







 

%From Figure \ref{fig:theoretical_analysis} middle, when the dataset size is smaller than $2^{11}$, different diffusion model shows the reproducible phenomenon. This is identifiable because all architectures converge to the same theoretical results. But what's more interesting is that when the dataset size is between $2^{11}$ and $2^{14}$, the reproducible phenomenon disappears, and when the dataset size is larger than $2^{14}$, the reproducible phenomenon appears again with even higher reproducibility score. This indicates that when the dataset size is large enough, the diffusion model does have enough capacity to converge to the theoretical solution but converges to another very similar score function, and it is still a unique encoding. This stage is a more interesting question because most of the diffusion model works in this situation where capacity is insufficient. However, identifying this stage is still an open question.

%Interestingly, we find a relation between our work and recent work \cite{yoon2023diffusion}. We reproduce their main results in Figure \ref{fig:theoretical_analysis} right. They find that when the model capacity is not enough (more training data and fewer model parameters), the diffusion model starts to generalize. We find that the stage of generalization is in coincidence with the stage of reproducibility. When dataset size is smaller than $2^{11}$, as we know diffusion mode has enough capacity to converge to the theoretical solution. And from \cite{somepalli2023understanding}, the optimal regression function doesn't have generalizability. So the duplication scores for different architectures are almost 1.0 in this stage. When the dataset size is between $2^{11}$ and $2^{14}$, the generalizability for architectures increase and the reproducibility decrease. And when the dataset size is larger than $2^{14}$, there is almost no duplication for generation and the reproducibility appears again. We think there should be a relation between the generalizability and reproducibility of the diffusion model.





%\subsection{Experimentical Verification}


